Maximizing Extractable Value from Automated Market Makers

Automated Market Makers (AMMs) are decentralized applications that allow users to exchange crypto-tokens without the need for a matching exchange order. AMMs are one of the most successful DeFi use cases: indeed, major AMM platforms process a daily volume of transactions worth USD billions. Despite their popularity, AMMs are well-known to suffer from transaction-ordering issues: adversaries can influence the ordering of user transactions, and possibly front-run them with their own, to extract value from AMMs, to the detriment of users. We devise an effective procedure to construct a strategy through which an adversary can maximize the value extracted from user transactions.

==> Makefile <==
SHELL := /bin/bash

# Files not managed by latex-make
SVG_FILES =

SVG_PDFT_FILES =

DOT_CIRCO_FILES =

DOT_DOT_FILES =

DOT_NEATO_FILES =

DOT_PATCHWORK_FILES =

DOT_FILES = $(DOT_CIRCO_FILES) $(DOT_DOT_FILES) $(DOT_NEATO_FILES) $(DOT_PATCHWORK_FILES)

PDF_FILES = \
	$(SVG_FILES:.svg=.pdf) \
	$(SVG_PDFT_FILES:.svg=.pdf) \
	$(DOT_FILES:.dot=.pdf)

GEN_TEX_FILES = $(DOT_TEX_FILES:.dot=.tex)

PDFT_FILES = $(SVG_PDFT_FILES:.svg=.svgpdft)

## Default target first
all: main.pdf

# Clear out all suffixes
#.SUFFIXES:
# List only those we will actually use
#.SUFFIXES: .pdf .svg .dot .tex .svgpdft

## Conversion from SVG files
%.pdf : %.svg.pdf
	inkscape --without-gui --export-area-drawing --export-pdf=$@ $<

## Conversion from SVG files
%.svgpdft : %.svg
	inkscape --without-gui --export-area-drawing \
	--export-pdf=$(basename $<).pdf --export-latex $<
	mv $(basename $<).pdf_tex $(basename $<).svgpdft

## Conversion from DOT files
$(DOT_CIRCO_FILES:.dot=.pdf) : $(DOT_CIRCO_FILES)
	circo -T pdf -o $@ $(basename $@).dot
$(DOT_DOT_FILES:.dot=.pdf) : $(DOT_DOT_FILES)
	dot -T pdf -o $@ $(basename $@).dot
$(DOT_NEATO_FILES:.dot=.pdf) : $(DOT_NEATO_FILES)
	neato -T pdf -o $@ $(basename $@).dot
$(DOT_PATCHWORK_FILES:.dot=.pdf) : $(DOT_PATCHWORK_FILES)
	patchwork -T pdf -o $@ $(basename $@).dot

$(DOT_TEX_FILES:.dot=.tex) : $(DOT_TEX_FILES)
	dot2tex --figonly -tmath $(basename $@).dot > $@

# Latex-make stuff follows

FIGURES = $(PDF_FILES) $(PDFT_FILES) $(GEN_TEX_FILES)

LU_FLAVORS = PDF

# Some flags required e.g. by the minted package
# PDFLATEX_OPTIONS += --shell-escape

# We require latex-make
include LaTeX.mk

# Loop target, for automatic rebuilding when a dependency file is updated
loop:
	./ifchanged.py $(TD_main.pdf_INPUTS) $(FIGURES) 'make'

## Additional cleanups
clean::
	rm -f $(PDF_FILES) $(PDFT_FILES)

arxiv::
	mkdir arxiv
	cp *.tex arxiv
	cp *.sol arxiv
	cp llncs.cls arxiv
	cp main.bbl arxiv
	cp splncs03.bst arxiv
	cp -r results arxiv
	cd arxiv; zip -r arxiv.zip .; mv arxiv.zip ..
#	rm -rf arxiv


==> bounded-blocks.tex <==
\subsection{Bounded blocks}
\label{sec:blockbound-swap-game}

We now study the mining game under the further assumption that
the number of transactions in a block is bounded by a given constant $n$, \ie
$|\bcB| \leq n$.


==> brute-force-swap.tex <==
\clearpage

\bigskip
\albertonote{*** BEGIN sketch of (very) brute-force algorithm I mentioned. It goes somewhere else (and may not be part of the paper). It is meant for the game where the miner has unlimited funds, no blocksize restriction and only swaps***}
\bigskip


 {\color{black!50} // Initial tentative solution is to do nothing} 

Let $\bcB_{\mathsf{sol}} = \epsilon$

 {\color{black!50} // Try all possible ways of discarding user transactions} 

For all sub-multisets  $\TxTi \subseteq \TxT$ 

\quad {\color{black!50} // Try all possible ways of ordering the user transactions} 

\quad For all permutations $\bcB$ of $\TxTi$ 

\quad \quad {\color{black!50} // Try all possible ways grouping the user transactions so as to create sandwich opportunities} 

\quad \quad For all possible decompositions of $\bcB_1 \dots \bcB_n= \bcB$

\quad \quad \quad Let $\bcBi = \epsilon$ and ${\confG}_0 = {\confG}$

\quad \quad \quad  {\color{black!50} // Try build the sequence of sandwiches} 

\quad \quad \quad For $i \in 1 \dots n$ 

\quad \quad \quad \quad Let $\txT$ and $\txTi$ be such that

\quad \quad \quad \quad ${\confG}_0 \myxrightarrow{\txT \bcBi_i \txTi} \confGi$ is the ``perfect sandwich'' 

\quad \quad \quad  \quad {\color{black!50} // CONJECTURE: The sandwich uniquely determined, and efficiently computable.} 

\quad \quad \quad \quad If the sandwich is not executable, break

\quad \quad \quad \quad {\color{black!50} Otherwise continue trying to build the sequence of sandwiches}

\quad \quad \quad \quad $\bcBi = \txT \bcB_i \txTi \bcBi$

\quad \quad \quad \quad ${\confG}_0 = {\confGi}$

\quad \quad \quad  {\color{black!50} // If the tentative solution is better, then save it} 

\quad \quad \quad If $\gain[\confG]{\pmvM}{\bcBi} \ge \gain[\confG]{\pmvM}{\bcB_{\mathsf{sol}}}$ then $\bcB_{\mathsf{sol}} = \bcBi $ 

{\color{black!50} // Return the best solution found} 

return $\bcB_{\mathsf{sol}}$

\bigskip

Main idea of completeness: (1) individual sandwiches are uniquely determined, (2) the only potential solutions in the space of possible solutions that is not being considered are sequences where miners have 3 or more consecutive swap operations. Regarding (2) note that this necessarily means that we would have 2 swaps int he same direction, which could be merged as just one swap operation. Regarding (1) my intuition is that the perfect sandwich is unique: do arbitrage before user, execute the user transactions, arbitrage again.

\bigskip
\albertonote{*** END ***}
\bigskip

\clearpage


==> cruft.tex <==
\begin{lemma}
  \label{lma:min-minted-price}
  Let $(\tokBal,\bcB)$ be a solution to the 0-txpool swap game
  in~$(\confG,\emptymset)$, where
  \mbox{$\confG = \mmid_{i \in I} (\ammR[i,0]:\tokT[i,0],\ammR[i,1]:\tokT[i,1]) \mid \confG[w]$}
  and $\confG[w]$ only contains user wallets.
  Let $\confG[0] = \walM{\tokBal} \mid \confG$.
  Let $\priceTx[\confG]{\tokT[0],\tokT[1]}{x}$ 
  be the price of $(\tokT[0],\tokT[1])$
  after performing a sequence of transactions $x$, \ie:
  \[
  \priceTx[\confG]{\tokT[0],\tokT[1]}{x}
  \; = \;
  \exchO[{\confG[x]}]{\tokT[0],\tokT[1]}
  \qquad
  \text{if \ $\confG[0] \myxrightarrow{x} \confG[x]$}
  \]
  Then, for all $i\in I$, 
  $\priceTx[\confG]{\tokT[i,0],\tokT[i,1]}{x}$
  is minimized by $\bcB$. \albertonote{I don't get what is meant by minimized by $\bcB$: function $p_{(\tokT[i,0],\tokT[i,1])}(x)$ has a single transaction as parameter. I guess this is the function that is being minimized but $\bcB$ is a transaction sequence, not a single transaction. Does the function need to be lifted to transaction sequences?}
\end{lemma}

Due to wealth conservation, the maximization of the miner's gain implies a maximization of the users loss: here, any change of the user's wealth must come from a change in token prices, since its balance remains constant throughout the game. Thus, a maximized miner gain implies minimized token prices for tokens present in user $\pmvA$'s wallet.

\albertonote{are the above properties inherent to this game or do they apply to other games?}



\Cref{lem:swaps-only} below establishes that deposits and redeems 
by the miner do not contribute any gain in the 0-txpool game.
Therefore, rational miners can neglect these transactions,
and only use $\ammSwapOp$ transactions in their solutions.
Thus, when solving the mining games greedily, the miner can achieve
an optimal result by without inserting redeem or deposit actions of its own into
the mining game solution.

\begin{lemma}
  \label{lem:swaps-only}
  Let $(\tokBal, \bcB)$ be a solution to the mining game in $(\confG,\TxT)$.
  Let $\txT$ be a transaction such that
  $\txType{\txT} \in \setenum{\ammDepositOp,\ammRedeemOp}$, and:
  \[
  \walM{\tokBal} \mid \confG \; \myxrightarrow{\txT} \; \walM{\cdots}\mid \confGi 
  \]
  If $(\tokBali, \bcBi)$ is a solution to the game in $(\confGi,\TxT)$, then:
  \[
    \gain[{\walM{\tokBal}\mid\confG}]{\pmvM}{\ \bcB} 
    \; = \;
    \gain[\walM{\tokBali}\mid{\confGi}]{\pmvM}{\ \txT \ \bcBi}
  \]
  \bartnote{I think this is false, because deposits change the swap values}
\end{lemma}
\begin{proof}
  Let $\confG[0] = \walM{\tokBali}\mid{\confGi}$, and 
  let $\confGi[0]$ be such that $\confG[0] \myxrightarrow{\txT} \confGi[0]$.
  By Lemma~3 in~\cite{ammTheory}, we have that
  $W_{\pmvA}(\confG[0]) = W_{\pmvA}(\confGi[0])$, \ie $\txT$ does not
  affect the net worth of any user (including $\pmvM$).
  Therefore:
  \[
  g' 
  \; \eqdef \;
  \gain[\walM{\tokBali}\mid{\confGi}]{\pmvM}{\ \txT \ \bcBi}
  \; = \;
  \gain[\walM{\tokBali}\mid{\confGi}]{\pmvM}{\ \bcBi}
  \]
  By contradiction, assume that
  $g \eqdef \gain[{\walM{\tokBal}\mid\confG}]{\pmvM}{\ \bcB} \neq g'$.
  If $g > g'$, then $(\tokBali,\bcBi)$ cannot be a solution in 
  $(\confGi,\TxT)$.
  \bartnote{rough idea: we can perform the same moves in $\bcB$, re-scaling the amounts. Note: the scaling factor is not constant: it depends on the transaction (and perhaps also on the whole history)}
  If $g < g'$, then $(\tokBal,\bcB)$ cannot be a solution in 
  $(\confG,\TxT)$.
  \bartnote{rough idea: we can perform the same moves in $\bcBi$, re-scaling the amounts}
\end{proof}


\bartnote{WIP: I do not think the theorem below can be proved without
referring to the construction of the optimal strategy}

Although the optimization of mining value extraction is rational at each mining round, we note that for a given set of user transactions $\TxT$, the extractable value value will also depend on the state $\confG$.
In particular, the miner with a higher balance of tokens may have the opportunity to extract additional value from the mining game, as it can perform a wider range of transactions.

We investigate the existence of an upper bound of extractable value for the miner, which given a higher balance at the beginning of the round, would be unable to extract additional value.
To this purpose, we assume that miners do not hold minted tokens,
that AMMs contain initial tokens only, and that users and miners
can only perform swap actions.

\albertonote{Is the universal quantification of $\tokBali$ also subject 
to $\dom(\tokBali) \subseteq \TokU[0]$?}

\begin{theorem}
  \label{th:miner:bounded-tokbal}
  Let $\TxT$ be a multiset of users' transactions, and
  let $\confG$ be a blockchain state not including $\pmvM$'s wallet.
  Then, there exists $\tokBal$ such that $\dom(\tokBal) \subseteq \TokU[0]$
  and, for all $\tokBali$:
  \[
  \mev{\walM{\tokBal} \mid \confG}{\TxT}
  \; \geq \;
  \mev{\walM{\tokBali} \mid \confG}{\TxT}
  \]
\end{theorem}


==> mev.tex <==
\section{Supplementary material}
\label{app}

\subsection{A basic example}
\label{sec:amm:ex}

\begin{figure}[b]
  \small
  \scalebox{0.95}{\parbox{\textwidth}{%
      \begin{align}
        % \nonumber
        % & \walA{70:\tokT[0], 80:\tokT[1]} \mid
        %   \walB{30:\tokT[0]}
        % \\
        % \label{ex:amm:xfer}
        % \xrightarrow{\actTransfer{\pmvA}{\pmvB}{10:\tokT[1]}} \;
        \nonumber
        & \walA{70:\tokT[0], 70:\tokT[1]} \mid
          \walB{30:\tokT[0],10:\tokT[1]}
        \\
        \label{ex:amm:dep0}
        \xrightarrow{\actAmmDeposit{\pmvA}{70}{\tokT[0]}{70}{\tokT[1]}} \;
        & \walA{70:(\tokT[0],\tokT[1])} \mid
          \walB{\cdots} \mid
          (70:\tokT[0],70:\tokT[1])
        \\
        \label{ex:amm:swapL}
        \xrightarrow{\actAmmSwapL{\pmvB}{30}{\tokT[0]}{20}{\tokT[1]}} \;
        & \walA{\cdots} \mid
          \walB{0:\tokT[0],31:\tokT[1]} \mid
          (100:\tokT[0],49:\tokT[1])
        \\
        \label{ex:amm:swapR}
        \xrightarrow{\actAmmSwapR{\pmvB}{29}{\tokT[0]}{21}{\tokT[1]}} \;
        & \walA{\cdots} \mid
          \walB{30:\tokT[0],10:\tokT[1]} \mid
          (70:\tokT[0],70:\tokT[1])
        \\
        \label{ex:amm:rdm}
        \xrightarrow{\actAmmRedeem{\pmvA}{30:(\tokT[0],\tokT[1])}} \;
        & \walA{30:\tokT[0],30:\tokT[1],40:(\tokT[0],\tokT[1])} \mid
          \walB{\cdots} \mid
          (40:\tokT[0],40:\tokT[1])
        \\
        \label{ex:amm:swapL1}
        \xrightarrow{\actAmmSwapL{\pmvB}{30}{\tokT[0]}{16}{\tokT[1]}} \;
        & \walA{\cdots} \mid
          \walB{0:\tokT[0],27:\tokT[1]} \mid
          (70:\tokT[0],23:\tokT[1])
        \\
        \label{ex:amm:rdm1}
        \xrightarrow{\actAmmRedeem{\pmvA}{30:(\tokT[0],\tokT[1])}} \;
        & \walA{82:\tokT[0],47:\tokT[1],10:(\tokT[0],\tokT[1])} \mid
          \walB{\cdots} \mid
          (18:\tokT[0],6:\tokT[1])
      \end{align}}}%
  \vspace{-10pt}
  \caption{Interactions between two users and an AMM.}
  \label{fig:amm}
\end{figure}


\Cref{fig:amm} displays a sequence of transitions.
%
% In step~\eqref{ex:amm:xfer},
% $\pmvA$ transfers \mbox{$10:\tokT[1]$} from her wallet to $\pmvB$'s.
%
In step~\eqref{ex:amm:dep0},
$\pmvA$ creates a new AMM, depositing
\mbox{$70:\tokT[0]$} and \mbox{$70:\tokT[1]$};
in return, she receives $70$ units of the minted token $(\tokT[0],\tokT[1])$.
%
In step~\eqref{ex:amm:swapL},
$\pmvB$ swaps $30$ of his units of $\tokT[0]$ for \emph{at least}
$20$ units of $\tokT[1]$.
The actual amount of units of $\tokT[1]$ received by $\pmvB$
is {\color{magenta}{$21$}}:
% , which regulates the relation between the state of the AMM before
% and after a swap, namely the product of the amount of both token types
% in the pair must remain constant,
indeed, $(70+30) \cdot (70-{\color{magenta}{21}}) = 70 \cdot 70$,
hence $21$ satisfies the constant product swap invariant.
% $\pmvB$ deposits $5$ units of $\tokT[0]$ and $\tokT[1]$ into the
% previously created AMM, receiving in return $5$ units of the minted token.
%
In step~\eqref{ex:amm:swapR},
$\pmvB$ reverses his prior action by swapping $21$ of his units of $\tokT[1]$ for \emph{at least}
$29$ units of $\tokT[0]$.
Here, the actual amount of units of $\tokT[1]$ received by $\pmvB$
is {\color{magenta}{$30$}}, which also satisfies the constant product swap invariant.
%
In step~\eqref{ex:amm:rdm},
$\pmvB$ redeems $30$ units of the minted token $(\tokT[0],\tokT[1])$,
accordingly reducing the funds in the AMM.
Note that the received tokens exhibit the same 1-to-1 ratio as in
the initial deposit at step~\eqref{ex:amm:dep0}.
%
In step~\eqref{ex:amm:swapL1},
$\pmvB$ swaps $30$ of his units of $\tokT[0]$ for \emph{at least}
$16$ units of $\tokT[1]$.
Unlike in the previous swap at step~\eqref{ex:amm:swapL},
now the actual amount of $\tokT[1]$ received by $\pmvB$ is $17$.
Note that the implied \emph{swap rate} between
received $\tokT[1]$ units and sent $\tokT[0]$ units
has deteriorated \wrt step~\eqref{ex:amm:swapL},
even if the pair $(\tokT[0],\tokT[1])$ had the same 1-to-1 ratio of funds.
%
Finally, in step~\eqref{ex:amm:rdm1}
$\pmvA$ performs another redeem of $30$ units of the minted token
$(\tokT[0],\tokT[1])$, thereby extracting $52$ units of $\tokT[0]$
and $17$ units of $\tokT[1]$ from the AMM.
Note that the ratio of redeemed tokens is no longer 1-to-1 as
in the previous redeem action~\eqref{ex:amm:rdm},
as the prior left swap has changed the ratio between the
funds of $\tokT[0]$ and $\tokT[1]$ in the AMM.
% This is less than user $\pmvB$'s original balance of $100:\tokT[0]$ due to the reduced reserves caused by the preceding redeem transaction.


\subsection{Variants of the mining game}
\label{sec:miner:variants}

\jamesnote{Previously in miner.tex}
The version of the mining game presented above is quite general,
as it does not constrain the number of miner and user transactions,
the number of AMMs in the state,
and the amount of tokens in wallets.
By adding constraints on the initial state and on the solution,
we can obtain several meaningful variants of the game.
We systematize below these variants,
by providing a taxonomy of mining games along four features.


\mypar{Miner balance}

In the general mining game,
the solution includes an initial miner balance $\tokBal$,
which is one of the two parameters against which the solution
maximizes the MEV.
In practice, this means that we assume
miners to have an unbounded availability of atomic tokens.
This assumption is not completely unrealistic,
as the miner can exchange its assets for atomic tokens,
and deposit these tokens to obtain minted tokens by the AMMs.
Further, miners can temporarily increase their balance
by \emph{flash loans}~\cite{qin2020attacking,wang2020towards},
which are incorporated in main AMM platforms like Uniswap~\cite{uniswapflash}.
%
We call \keyterm{balance-bounded} the variants of the game
where we assume that the miner balance is fixed \emph{a priori}.
Formally, the initial blockchain state $\confG$ now contains
a given miner wallet $\walM{\tokBal}$,
and the move of the game is just a block $\bcB$.
In this variant, the solution to the game must maximize
the one-variable function
\(
\gain[\confG]{\pmvM}{y}
\),
and the maximum extractable value in $(\confG,\TxT)$
is defined accordingly as
\(
\mev{\confG}{\TxT} = \gain[\confG]{\pmvM}{\bcB}
\),
where $\bcB$ is a solution to the game.


\mypar{Number of AMMs}

In the general game, the initial blockchain state $\confG$ may contain
an arbitrary number of AMMs.
We call \keyterm{1-AMM} the variant of the mining game
where all the actions in the solution $\bcB$ target a single AMM.
This variant is still worth of study,
because it may allow to solve the general problem
in two phases: first, compute the  solution for each individual AMM,
and then greedily apply the locally-optimal move to each AMM.
We show an instance of this approach in~\Cref{sec:0txpool-game}.


\mypar{Size of txpool}

In the general game, the txpool $\TxT$ can contain an arbitrary (finite)
multiset of user transactions.
Two relevant subcases are when the $\TxT$ is empty
(called \keyterm{0-txpool}), and when it contains exactly one transaction
(\keyterm{1-txpool}).
The 0-txpool variant is a generalization of the so-called
\emph{arbitrage problem}, which has been studied before
in~\cite{angeris2019analysis,Angeris20improvedoracles}
in the restricted setting where players can only perform $\ammSwapOp$ actions,
and in~\cite{ammTheory} under an abstract notion of swap invariant.
% \bartnote{check if~\cite{angeris2019analysis} uses the same hypothesis
The 1-txpool case is the basis for greedy approaches trying to solve
the mining game transaction-by-transaction.
We show an instance of this approach in~\Cref{sec:ntxpool-game}.


\mypar{Number of transactions in a block}

In the general game, the sequence $\bcB$ in the solution
can contain an arbitrary number of transactions.
In practice, blockchain platforms usually impose a limit to the size
of blocks.
We can model this constraint
by bounding the size of $\bcB$ to a given constant $n$.
Although this variant makes finding exact solutions to the game more complex,
it is still possible to use the solution of the unbounded-block game
as a \emph{sub-optimal} solution of the bounded-block variant,
\ie the bounded sequence $\bcB$ increases $\pmvM$'s gain,
but not in an optimal way (see~\Cref{th:bounded-block-suboptimal}).


\section{Solving the mining game}
\label{sec:mev}

\begin{center}
\begin{figure*}[t]
{\tiny
  \begin{tikzcd} [sep = .15 cm]
  %
    & \stackrel{\textbf{k-AMM, 0-txpool, $\infty$-balance}}{\S~\ref{sec:0txpool-game}} \arrow [dd, color=black!50, dotted]  \arrow [dl, color=black!50, dotted]  & & \stackrel{\textbf{k-AMM, 1-txpool, $\infty$-balance}}{\S~\ref{sec:1txpool-game}} \arrow [dd, color=black!50, dotted] \arrow [ll, color=black!50, dotted] \arrow [dl, color=black!50, dotted] & & \stackrel{\textbf{k-AMM, n-txpool, $\infty$-balance}}{\stackrel{\text{(general mining game)}}{\S~\ref{sec:ntxpool-game}}}\arrow [dd, color=black!50, dotted]  \arrow [ll, color=black!50, dotted] \arrow [dl, color=black!50, dotted]  \\
    %
    {\color{black!50}\text{k-AMM, 0-txpool, bounded-balance}} \arrow [dd, color=black!50, dotted] & & {\color{black!50}\text{k-AMM, 1-txpool, bounded-balance}} \arrow [dd, color=black!50, dotted]  \arrow [ll, color=black!50, dotted]  & &  {\color{black!50}\text{k-AMM, n-txpool, bounded-balance}} \arrow [dd, color=black!50, dotted] \arrow [ll, color=black!50, dotted] & \\
    %
    & \stackrel{\textbf{1-AMM, 0-txpool, $\infty$-balance}}{\S~\ref{sec:1amm-0txpool-game}} \arrow [dl, color=black!50, dotted] & & {\color{black!50}\text{1-AMM, 1-txpool, $\infty$-balance}} \arrow [ll, color=black!50, dotted] \arrow [dl, color=black!50, dotted] & & {\color{black!50}\text{1-AMM, n-txpool, $\infty$-balance}} \arrow [ll, color=black!50, dotted] \arrow [dl, color=black!50, dotted] \\
    \stackrel{\textbf{1-AMM, 0-txpool, bounded-balance}}{\S~\ref{sec:balbound-1amm-1txpool-game}} & & {\color{black!50}\text{1-AMM, 1-txpool, bounded-balance}} \arrow [ll, color=black!50, dotted] & & {\color{black!50}\text{1-AMM, n-txpool, bounded-balance}} \arrow [ll, color=black!50, dotted]
  \end{tikzcd}
}
\caption{Variants of the mining game: ``$x$-AMM, $y$-txpool, $z$'' indicates a game with $x$ AMMs, a txpool of size $y$, and where the miner wallet is $z$ (bounded or unbounded).
%
Some variants are labelled with the subsection where their solution is provided. Arrows relate games by their relative restrictions (the target game has more constraints than the source game). }
\label{fig:gamespace}
\end{figure*}
\end{center}

Solving the mining game through an exhaustive search of the optimal move
is not possible:
indeed, even assuming that the number of transactions in $\bcB$ is bounded,
the state space is unbounded,
since the actual parameters of $\pmvM$'s transactions are
chosen from an infinite set.
%
In this~\namecref{sec:mev} we construct solutions to the mining game,
both in its general form and in some relevant variants.
\Cref{fig:gamespace} provides an overview of the games we consider.
%The order of presentation does not follow the order of generality; it provides an incremental presentation for the benefit of the reader.
%
% To the best of our knowledge, there are no efficient algorithms
% to solve the general mining game.
%
% Therefore, even if we study the general mining game in this paper, it is also important to study specific variants of it, as we do.


\subsection{1-AMM,  0-txpool game}
\label{sec:1amm-0txpool-game}

We recall that in this variant of the game,
the miner can operate on a \emph{single} AMM,
and there are no transactions in the txpool.
%
In order to construct a solution to this game
(\Cref{th:1amm-1txpool-game}),
we need some auxiliary definitions.
Let $\tokT[0],\tokT[1]$ be atomic token types,
% let $\tokBal$ be a balance,
and let $\confG$ be a state
with $\res[{\tokT[0],\tokT[1]}](\confG) = (\ammR[0],\ammR[1])$.
For each swap direction $d \in \setenum{0,1}$,
we define the \keyterm{canonical swap values} as:
\begin{align*}
  \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{}
  & = \sqrt{\tfrac{\exchO{\tokT[1-d]}}{\exchO{\tokT[d]}} \cdot \ammR[0] \cdot \ammR[1]} - \ammR[d]
  \\
  \swapVal[1-d]{d}{\tokT[0],\tokT[1]}{\confG}{}
  & = \frac
    {\ammR[1-d] \cdot \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{}}
    {\ammR[d] + \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{}}
\end{align*}

Intuitively, these values define the amount of tokens to be exchanged
when the solution to the game is indeed a swap of tokens.
The value $\swapVal[d]{d}{}{}{}$ is the amount of tokens deposited
in a swap of direction $d$: it is defined in such a way
that, after the swap, the AMM reaches an equilibrium, where
the ratio of the AMM reserves is equal to
the (inverse) ratio of the token prices.
The value $\swapVal[1-d]{d}{}{}{}$ is the amount of tokens received back
after the swap, and it is computed as a function of
$\swapVal[d]{d}{}{}{}$: it is the unique value for which the swap
invariant is satisfied.
If a swap direction $d$ satisfies:
\[
\swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{} > 0
% \qquad
% \swapVal[1-d]{d}{\tokT[0],\tokT[1]}{\confG}{} > 0
\]
then we define the \keyterm{canonical swap transaction} (a potential solution to the game, as we shall see) as:
\[
\actAmmSwap
{\pmvM}
{d}
{\swapVal[0]{d}{\tokT[0],\tokT[1]}{\confG}{}}{\tokT[0]}
{\swapVal[1]{d}{\tokT[0],\tokT[1]}{\confG}{}}{\tokT[1]}
\]
and we denote this transaction by
$\swapTx{\tokT[0],\tokT[1]}{\confG}{}$.
%
When we want to remark that $d$ is the swap direction,
we write $\swapTx[d]{\tokT[0],\tokT[1]}{\confG}{}$.

\begin{lemma}
  \label{lem:swapTx:enabled}
  If the canonical swap transaction $\swapTx[d]{\tokT[0],\tokT[1]}{\confG}{}$
  is defined,
  then it is enabled in $\walM{\tokBal} \mid \confG$ whenever
  $\tokBal(\tokT[d]) \geq \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{}$.
\end{lemma}
\begin{proof}
  Let $\valV[d] = \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{}$
  let $\valV[1-d] = \swapVal[1-d]{d}{\tokT[0],\tokT[1]}{\confG}{}$,
  and let $\confG[0] = \walM{\tokBal} \mid \confG$.
  The assumption $\tokBal(\tokT[d]) \geq \valV[d]$ guarantees that
  $\pmvM$ has enough balance of $\tokT[d]$ to deposit to the AMM.
  So, we just need show that the swap values respect the
  premise of rule~\nrule{[Swap]} , \ie:
  \[
  \valV[1-d] \leq \frac{\ammR[1-d] \cdot \valV[d]}{\ammR[d]+\valV[d]}
  \]
  This follows directly by the definition of
  $\swapVal[1-d]{d}{\tokT[0],\tokT[1]}{\confG}{}$.
\end{proof}

\begin{example}
  \label{ex:1amm-1txpool-game}
  Let \mbox{$\confG = (18:\tokT[0],6:\tokT[1])$},
  and let the prices of the atomic tokens be
  $\exchO{\tokT[0]} = 5$ and $\exchO{\tokT[1]} = 9$.
  We have that:
  \begin{align*}
    % \valV[0]^0
    % =
    % \swapVal[0]{0}{\tokT[0],\tokT[1]}{\confG}{\tokBal}
    % & = \sqrt{\frac{9}{5} \cdot \ammR[0] \ammR[1]} - \ammR[0]
    % =
    % \sqrt{\frac{9}{5} \cdot 18 \cdot 6} - 18
    % \approx
    % -2
    % \\
    % \valV[1]^0
    % =
    % \swapVal[1]{0}{\tokT[0],\tokT[1]}{\confG}{\tokBal}
    % & =
    % \frac{\ammR[1] \valV[0]^0}{\ammR[0] + \valV[0]^0}
    % =
    % \frac{6 \cdot (-2)}{18 - 2}
    % =
    % -0.75
    % \\
    \swapVal[1]{1}{\tokT[0],\tokT[1]}{\confG}{}
      & =
        \sqrt{\frac{5}{9} \cdot 18 \cdot 6} - 6
        \approx
        1.75
    \\
    \swapVal[0]{1}{\tokT[0],\tokT[1]}{\confG}{}
      & =
        \frac{18 \cdot 1.75}{6 + 1.75}
        \approx
        4
  \end{align*}
  The canonical swap transaction is
  \(
  \txT
  =
  \actAmmSwap{\pmvM}{1}{4}{\tokT[0]}{1.75}{\tokT[1]}
  \).
  We anticipate that,
  by~\Cref{th:1amm-1txpool-game}, the solution of the mining game
  is $(\tokBal,\txT)$, for any $\tokBal$
  such that $\tokBal(\tokT[1]) \geq 1.75$
  and $\tokBal(\tokT[0],\tokT[1]) = 0$.
  Since $\tokBal$ has enough units of $\tokT[1]$ to perform
  the right swap, $\pmvM$ can fire $\txT$ from $\walM{\tokBal} \mid \confG$,
  reaching the state:
  \[
  % \confG[\ref{ex:amm:rdm1}]
  % \xrightarrow{\actAmmSwapR{\pmvA}{3}{\tokT[0]}{2}{\tokT[1]}} \;
  \walM{\tokBal - 1.75:\tokT[1] + 4:\tokT[0]} \mid
  (14:\tokT[0],7.75:\tokT[1])
  \]
  In this state, the AMM has reached an equilibrium,
  where the ratio of the reserves equals to the (inverse) ratio of the token prices:
  \[
  \frac{14}{7.75} \; = \; 1.8 \; = \; \frac{\exchO{\tokT[1]}}{\exchO{\tokT[0]}}
  \]
  The gain of $\pmvM$ after this step is:
  % the canonical swap gain:
  \[
  (4 \cdot 5 - 1.75 \cdot 9)
  \; \cdot \;
  \Big(
  1 - \frac{\tokBal(\tokT[0],\tokT[1])}{\supply{(\tokT[0],\tokT[1])}(\confG)}
  \Big)
  \]
  Note that requiring $\tokBal(\tokT[0],\tokT[1]) = 0$
  ensures that this gain is maximized (to $4.57$).
  Any other choice would result in a lower gain for $\pmvM$.
  %\albertonote{Question not related to this game: Does this mean that if a miner is allowed to do other tokens (a different game) and he/she has minted tokens she should first redeem them?} \bartnote{yes}
  \qed
\end{example}

The following~\namecref{lem:swapTx:mutual-exclusion}
establishes that swap directions are mutually exclusive:
if the deposited canonical value for direction $d$ is positive
(\ie, $\swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{} > 0$),
then the value for the opposite direction is negative
(\ie, $\swapVal[d]{1-d}{\tokT[0],\tokT[1]}{\confG}{}$ < 0),
and \emph{vice versa}.
Further, the deposited and redeemed canonical values for the same direction
have the same sign.
Hence, if a swap transaction with the canonical values
is enabled in a given direction $d$, then
the transaction in the opposite direction is not enabled,
because its values are negative.
The~\namecref{lem:swapTx:mutual-exclusion} also states
that if a swap value in a given direction is zero,
then also the values in the other direction are zero.

\begin{lemma}
  \label{lem:swapTx:mutual-exclusion}
  For $\circ \in \setenum{=,>}$:
  \[
  \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{} \circ 0
  \iff
  \swapVal[1-d]{d}{\tokT[0],\tokT[1]}{\confG}{} \circ 0
  \;\; \text{and} \;\;
  0 \circ \swapVal[1-d]{1-d}{\tokT[0],\tokT[1]}{\confG}{}
  \]
\end{lemma}

The following~\namecref{lem:swapTx:gain} quantifies
the gain of $\pmvM$ upon firing a swap transaction
(not necessarily the canonical one).
% $\swapTx[d]{\tokT[0],\tokT[1]}{\confG}{}$
% with swap direction $d$
% in state $\walM{\tokBal} \mid \confG$ .

\begin{lemma}[Swap gain]
  \label{lem:swapTx:gain}
  % For all $\tokT[0],\tokT[1] \in \TokU[0]$, and
  For all $\confG[0] = \walM{\tokBal} \mid \confG$ such that the transaction
  \(
  \txT =
  % \swapTx[d]{\tokT[0],\tokT[1]}{\confG}{}
  % \; = \;
  \actAmmSwap{\pmvM}{d}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}
  \)
  is enabled in $\confG[0]$:
  \begin{align*}
    & \gain[{\confG[0]}]{\pmvM}{\txT}
      =
      \big(
      \valV[1-d] \ \exchO{\tokT[1-d]}
      -
      \valV[d] \ \exchO{\tokT[d]}
      \big)
      %
      \Big(
      1 - \frac{\tokBal(\tokT[0],\tokT[1])}{\supply{(\tokT[0],\tokT[1])}(\confG[0])}
      \Big)
  \end{align*}
\end{lemma}
\begin{proof}
  Let $\confG[0] = \walM{\tokBal} \mid \confG$,
  let $\txT = \actAmmSwap{\pmvM}{d}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}$
  % $\txT = \swapTx[d]{\tokT[0],\tokT[1]}{\confG}{}$,
  and let $\confGi[0]$ be such that $\confG[0] \myxrightarrow{\txT} \confGi[0]$.
  Let $\res[{\tokT[0],\tokT[1]}](\confG) = (\ammR[0],\ammR[1])$.
  % The canonical swap transaction has the form:
  % \[
  % \actAmmSwap{\pmvM}{d}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}
  % \]
  % where
  % $\valV[i] = \swapVal[i]{d}{\tokT[0],\tokT[1]}{\confG}{}$
  % for $i \in \setenum{0,1}$.
  By~\eqref{def:gain:A}:
  \[
  \gain[\walM{\tokBal} \mid \confG]
  {\pmvM}
  {\txT}
  \; = \;
  W_{\pmvM}(\confGi[0]) - W_{\pmvM}(\confG[0])
  \]
  By definition of net worth~\eqref{eq:net-worth:user}, we have that:
  \begin{align*}
    W_{\pmvM}(\confG[0])
    & = \tokBal(\tokT[d]) \cdot \exchO{\tokT[d]}
      + \tokBal(\tokT[1-d]) \cdot \exchO{\tokT[1-d]}
    \\
    & + \tokBal(\tokT[0],\tokT[1])
      \cdot \dfrac
      {\ammR[d] \cdot \exchO{\tokT[d]} + \ammR[1-d] \cdot \exchO{\tokT[1-d]}}
      {\supply{(\tokT[0],\tokT[1])}(\confG[0])}
    \\
    & + \textstyle \sum_{\tokT \not\in \setenum{\tokT[0],\tokT[1], (\tokT[0],\tokT[1])}}
      \tokBal(\tokT) \cdot \exchO[{\confG[0]}]{\tokT}
    \\
    W_{\pmvM}(\confGi[0])
    & = (\tokBal(\tokT[d]) - \valV[d]) \cdot \exchO{\tokT[d]}
      + (\tokBal(\tokT[1-d]) + \valV[1-d]) \cdot \exchO{\tokT[1-d]}
    \\
    & + \tokBal(\tokT[0],\tokT[1])
      \cdot \dfrac
      {(\ammR[d] + \valV[d]) \cdot \exchO{\tokT[d]} + (\ammR[1-d] - \valV[1-d]) \cdot \exchO{\tokT[1-d]}}
      {\supply{(\tokT[0],\tokT[1])}(\confG[0])}
    \\
    & + \textstyle \sum_{\tokT \not\in \setenum{\tokT[0],\tokT[1], (\tokT[0],\tokT[1])}}
      \tokBal(\tokT) \cdot \exchO[{\confGi[0]}]{\tokT}
  \end{align*}
  Since $\exchO[{\confG[0]}]{\tokT} = \exchO[{\confGi[0]}]{\tokT}$
  for all $\tokT \not\in \setenum{\tokT[0],\tokT[1], (\tokT[0],\tokT[1])}$,
  it follows that:
  \begin{align*}
    & W_{\pmvM}(\confGi[0]) - W_{\pmvM}(\confG[0])
    \\
    & = \valV[1-d] \cdot \exchO{\tokT[1-d]}
      - \valV[d] \cdot \exchO{\tokT[d]}
      + \frac
      {\valV[d] \cdot \exchO{\tokT[d]} - \valV[1-d] \cdot \exchO{\tokT[1-d]}}
      {\supply{(\tokT[0],\tokT[1])}(\confG[0])}
    \\
    & = \big( \valV[1-d] \cdot \exchO{\tokT[1-d]} - \valV[d] \cdot \exchO{\tokT[d]} \big)
      \Big( 1 - \frac{1}{\supply{(\tokT[0],\tokT[1])}(\confG[0])} \Big)
      \qed
  \end{align*}
\end{proof}


We are now ready to construct the solution to the 1-AMM, \mbox{0-txpool} game.
Intuitively, the optimal move is the canonical swap transaction when defined,
or otherwise it is just ``do nothing''.

\begin{theorem}
  \label{th:1amm-1txpool-game}
  Let \
  \mbox{$\confG = (\ammR[0]:\tokT[0],\ammR[1]:\tokT[1]) \mid \confG[w]$},
  where $\confG[w]$ only contains user wallets,
  and let $\TxT = \emptymset$.
  %
  If the canonical swap is undefined,
  then $(\tokBal,\emptyseq)$ is a solution to the game,
  for all $\tokBal$.
  %
  Otherwise,
  % if the canonical swap is
  % $\swapTx[d]{\tokT[0],\tokT[1]}{\confG}{\tokBal}$, then
  $(\tokBal,\swapTx[d]{\tokT[0],\tokT[1]}{\confG}{})$
  is a solution to the game,
  for all $\tokBal$ such that
  \(
  \tokBal(\tokT[d])
  \geq
  \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{}
  \)
  and
  $\tokBal(\tokT[0],\tokT[1]) = 0$.
  % bart: obvious from definition??
  % Further,
  % \(
  % \mev{\confG}{\TxT
  % =
  % \swapGainNew[\pmvM]{\tokT[0],\tokT[1]}{\confG}{\tokBal}
  % \).
\end{theorem}
\begin{proof}
  Let $\confG[0] = \walM{\tokBal} \mid \confG$,
  where $\tokBal$ respect the hypotheses in the statement.
  For all $x > 0$, let:
  \[
  \begin{array}{l}
    \txY^0(x)
    \; = \;
    \actAmmSwap{\pmvM}{0}{x}{\tokT[0]}{y_0}{\tokT[1]}
    \\[5pt]
    \txY^1(x)
    \; = \;
    \actAmmSwap{\pmvM}{1}{y_1}{\tokT[0]}{x}{\tokT[1]}
  \end{array}
  \quad
  y_d = \frac{\ammR[1-d] \cdot x}{\ammR[d]+x}
  \]
  Note that $\txY^d(x)$ is enabled in $\confG[0]$ for all $x$
  such that $\tokBal(\tokT[d]) \geq x$,
  since $y_d \leq \ammR[1-d]$ for all $x$.
  There are two cases, depending on whether the canonical swap
  $\txT = \swapTx[d]{\tokT[0],\tokT[1]}{\confG}{} = \actAmmSwap{\pmvM}{d}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}$
  is defined or not.
  If $\txT$ is defined, then the swap direction $d$ satisfies:
  \begin{equation*}
    \valV[d] = \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{} > 0
  \end{equation*}
  By definition of the canonical swap values, this implies:
  \begin{equation}
    \label{eq:1amm-1txpool-game:1}
    a
    \; \eqdef \;
    \ammR[1-d] \ \exchO{\tokT[1-d]} -  \ammR[d] \ \exchO{\tokT[d]}
    \; > \;
    0
  \end{equation}
  and, by~\Cref{lem:swapTx:mutual-exclusion}, it also follows that:
  \begin{equation*}
    \valV[1-d] = \swapVal[1-d]{d}{\tokT[0],\tokT[1]}{\confG}{} > 0
    \qquad
    \swapVal[1-d]{1-d}{\tokT[0],\tokT[1]}{\confG}{} < 0
  \end{equation*}
  We first show that $\txY^{1-d}(x)$ decreases $\pmvM$'s gain,
  for all $x$.
  Let $\tokBal$ be any balance without minted tokens,
  let $\confG[0] = \walM{\tokBal} \mid \confG$, and
  let $\confGi[x]$ be such that
  $\confG[0] \myxrightarrow{\txY^{1-d}(x)} \confGi[x]$.
  We have that:
  \begin{align*}
    \gain[{\confG[0]}]{\pmvM}{\txY^{1-d}(x)}
    & = W_{\pmvM}(\confGi[x]) - W_{\pmvM}(\confG[0])
    \\
    & = y_{1-d} \exchO{\tokT[d]} - x \exchO{\tokT[1-d]}
    \\
    & = \frac{\ammR[d] \cdot x}{\ammR[1-d]+x} \exchO{\tokT[d]} - x \exchO{\tokT[1-d]}
    \\
    & = \frac{\ammR[d] \ x \ \exchO{\tokT[d]} - x (\ammR[1-d]+x) \exchO{\tokT[1-d]}}{\ammR[1-d]+x}
    \\
    & = \frac{x \big( \ammR[d] \exchO{\tokT[d]} - \ammR[1-d]\exchO{\tokT[1-d]} \big) + x^2 \exchO{\tokT[1-d]}}{\ammR[1-d]+x}
    \\
    & = \frac{- a x - x^2 \exchO{\tokT[1-d]}}{\ammR[1-d]+x}
  \end{align*}
  By~\eqref{eq:1amm-1txpool-game:1} we have $a > 0$:
  therefore, $\gain[\pmvM]{\confG[0]}{\txY^{1-d}(x)} < 0$,
  \ie $\txY^{1-d}(x)$ decreases $\pmvM$'s gain, for all $x$.
  %
  We then show that the gain for $\pmvM$
  with the canonical swap transaction $\txT$
  is greater than any swap transaction with direction $d$, \ie
  for all $x > 0$:
  \[
  \gain[{\confG[0]}]{\pmvM}{\txT}
  \geq
  \gain[{\confG[0]}]{\pmvM}{\txY^{d}(x)}
  \]
  By~\Cref{lem:swapTx:gain},
  and using the assumption that $\tokBal(\tokT[0],\tokT[1])$:
  \begin{align*}
    \gain[{\confG[0]}]{\pmvM}{\txY^{d}(x)}
    & = y_d \ \exchO{\tokT[1-d]} - x \ \exchO{\tokT[d]}
    \\
    & = \frac{\ammR[1-d] \cdot x}{\ammR[d] + x} \ \exchO{\tokT[1-d]} - x \ \exchO{\tokT[d]}
    \\
    & = \frac{\ammR[1-d] \cdot x \ \exchO{\tokT[1-d]} - \ammR[d] \exchO{\tokT[d]} - x^2 \ \exchO{\tokT[d]}}{\ammR[d] + x}
    \\
    & = \frac{a x - x^2 \ \exchO{\tokT[d]}}{\ammR[d] + x}
  \end{align*}
  To find the maximum of $\gain[{\confG[0]}]{\pmvM}{\txY^{1-d}(x)}$,
  we find the point $x$ for which the derivative is $0$.
  We have that:
  \begin{align*}
    \frac{\partial}{\partial x} \gain[{\confG[0]}]{\pmvM}{\txY^{d}(x)}
    & = \frac
      {a \ \ammR[d] - \exchO{\tokT[d]} \ x \ (2 \ \ammR[d] + x)}
      {(\ammR[d] + x)^2}
  \end{align*}
  This derivative equals to zero if and only of:
  \begin{align*}
    x
    & = \sqrt{
      \frac
      {\ammR[d] \cdot (a + \ammR[d] \ \exchO{\tokT[d]})}
      {\exchO{\tokT[d]}}
      }
      - \ammR[d]
  \end{align*}
  By expanding the definition of $a$ in~\eqref{eq:1amm-1txpool-game:1}:
  \begin{align*}
    x
    & = \sqrt{
      \frac{\exchO{\tokT[1-d]}}{\exchO{\tokT[d]}} \cdot
      \ammR[d] \cdot \ammR[1-d]
      }
      \, - \, \ammR[d]
      \; = \;
      \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{}
  \end{align*}
  By~\Cref{lem:0txpool:swaps-only},
  we can restrict to sequences of $\ammSwapOp$ transactions.
  Then, the canonical swap transaction maximizes $\pmvM$'s gain.

  \medskip\noindent
  Otherwise, if $\txT$ is undefined, it must be
  $\swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{} = 0$
  for $d \in \setenum{0,1}$.
  By definition of the canonical swap values, this implies:
  \begin{equation}
    \label{eq:1amm-1txpool-game:1}
    a
    \; \eqdef \;
    \ammR[1-d] \ \exchO{\tokT[1-d]} -  \ammR[d] \ \exchO{\tokT[d]}
    \; = \;
    0
  \end{equation}
  For all $x \geq 0$, we have that:
  \[
  \gain[{\confG[0]}]{\pmvM}{\txY^{1-d}(x)}
  \; = \;
  \frac{- a x - x^2 \exchO{\tokT[1-d]}}{\ammR[1-d]+x}
  \; = \;
  \frac{- x^2 \exchO{\tokT[1-d]}}{\ammR[1-d]+x}
  \; \leq \;
  0
  \]
  Therefore, the empty move is a solution to the game.
\end{proof}


\subsection{Balance-bounded 1-AMM,  0-txpool game}
\label{sec:balbound-1amm-1txpool-game}

The solution of the balance-bounded variant of the game
is similar to that of~\Cref{th:1amm-1txpool-game},
except that now the canonical swap values
depend also on the initial miner's balance $\tokBal$.
Formally, let $\tokT[0],\tokT[1]$ be atomic token types,
let $\tokBal$ be a balance,
let $\confG$ be a state
with $\res[{\tokT[0],\tokT[1]}](\confG) = (\ammR[0],\ammR[1])$
and with $\walM{\tokBal} \in \confG$.
For each swap direction $d \in \setenum{0,1}$,
we define the \keyterm{bounded canonical swap values} as:
\begin{align*}
  \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{\tokBal}
  & =
    \min \Big\{
    \tokBal(\tokT[d]), \;
    \sqrt{\tfrac{\exchO[{\confG}]{\tokT[1-d]}}{\exchO[{\confG}]{\tokT[d]}} \cdot \ammR[0] \cdot \ammR[1]} - \ammR[d]
    \Big\}
  \\
  \swapVal[1-d]{d}{\tokT[0],\tokT[1]}{\confG}{\tokBal}
  & = \frac
    {\ammR[1-d] \cdot \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{\tokBal}}
    {\ammR[d] + \swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{\tokBal}}
\end{align*}

\noindent
If a swap direction $d$ satisfies the inequality:
\[
\swapVal[d]{d}{\tokT[0],\tokT[1]}{\confG}{\tokBal} > 0
% \qquad
% \swapVal[1-d]{d}{\tokT[0],\tokT[1]}{\confG}{\tokBal} > 0
\]
then we define the \keyterm{bounded canonical swap transaction} as:
\[
\actAmmSwap
{\pmvM}
{d}
{\swapVal[0]{d}{\tokT[0],\tokT[1]}{\confG}{\tokBal}}{\tokT[0]}
{\swapVal[1]{d}{\tokT[0],\tokT[1]}{\confG}{\tokBal}}{\tokT[1]}
\]
and we denote this transaction by
$\swapTx{\tokT[0],\tokT[1]}{\confG}{\tokBal}$.
When we want to remark that $d$ is the swap direction,
we write $\swapTx[d]{\tokT[0],\tokT[1]}{\confG}{\tokBal}$.


\begin{example}
  \label{ex:balbound-1amm-1txpool-game}
  Recall the state \mbox{$\confG = (18:\tokT[0],6:\tokT[1])$}
  from~\Cref{ex:1amm-1txpool-game},
  and now assume that the miner $\pmvM$ has an initial balance
  $\tokBal = \setenum{1:\tokT[0]}$.
  The bounded canonical swap transaction is:
  \[
  \actAmmSwap
  {\pmvM}
  {1}
  {2.57}{\tokT[0]}
  {1}{\tokT[1]}
  \]
  The gain of $\pmvM$ after firing this transaction is:
  \[
  2.57 \cdot \exchO{\txT[0]} - 1.75 \cdot \exchO{\txT[0]}
  \; = \;
  2.57 \cdot 5 - 1.75 \cdot 9
  \; = \;
  3.86
  \]
  Note that this gain is lower than $4.57$, \ie the gain obtained
  in the unbounded-balance case.
  \qed
\end{example}


\begin{theorem}
  \label{th:balbound-1amm-1txpool-game}
  Let \
  \mbox{$\confG = \walM{\tokBal} \mid (\ammR[0]:\tokT[0],\ammR[1]:\tokT[1]) \mid \confG[w]$},
  where $\confG[w]$ only contains user wallets,
  and let $\TxT = \emptymset$.
  %
  If the bounded canonical swap is undefined,
  then $\emptyseq$ is a solution to the game.
  %
  Otherwise,
  % if the canonical swap is
  % $\swapTx[d]{\tokT[0],\tokT[1]}{\confG}{\tokBal}$, then
  $\swapTx[d]{\tokT[0],\tokT[1]}{\confG}{\tokBal}$
  is a solution to the game.
  % bart: obvious from definition??
  % Further,
  % \(
  % \mev{\confG}{\TxT}
  % \leq
  % \swapGainNew[\pmvM]{\tokT[0],\tokT[1]}{\confG}{\tokBal}
  % \).
\end{theorem}



\subsection{0-txpool game}
\label{sec:0txpool-game}

We now generalise the solution constructed in~\Cref{sec:1amm-0txpool-game}
to the case where the miner can operate on multiple AMMs,
still assuming that the txpool is empty.
We construct the solution to this game by greedily solving the 1-AMM game
for each AMM in the state, and then composing the obtained solutions.
Below, we indicate with $\bcB \bcBi$ the concatenation of two sequences,
and with $\tokBal + \tokBal$ the composition of two balances, \ie
$(\tokBal + \tokBali)(\tokT)$ is the summation of the balance of $\tokT$
in $\tokBal$ and in $\tokBali$.

\begin{theorem}
  \label{th:0-txpool-swap-game:greedy}
  Let \
  \mbox{$\confG = \mmid_{i \leq n} (\ammR[i,0]:\tokT[i,0],\ammR[i,1]:\tokT[i,1]) \mid \confG[w]$}
  be such that $\confG[w]$ only contains user wallets.
  For all $j \in I$, let
  $(\tokBal[j],\bcB[j])$ be a solution to the 1-AMM game
  in $(\confG,\emptymset)$ such that
  $\pmvM$ only operates on the AMM pair $(\tokT[j,0],\tokT[j,1])$.
  % Let $\confG \myxrightarrow{\bcB} \confGi$.
  % If $(\tokBali,\bcBi)$ is a solution to the game in $(\confGi,\TxT)$,
  % then, $(\tokBal+\tokBali,\bcB\bcBi)$ is a solution to the game in $(\confG,\TxT)$.
  Then, $(\tokBal[1] + \cdots + \tokBal[n],\bcB[1] \cdots \bcB[n])$
  is a solution to the 0-txpool game in $(\confG,\emptymset)$.
\end{theorem}


% \begin{lemma}
%   \label{lma:price-minimization}
%   Let $(\tokBal,\bcB)$ be the 0-txpool game solution of $(\emptyset,\confG)$ where $\confG = \mmid_{i \in I} (\ammR[i,0]:\tokT[i,0],\ammR[i,1]:\tokT[i,1]) \mid \confG[w]$, $\confG[w]$ only contains user wallets. Furthermore, let $\walM{\tokBal}\mid\confG \rightarrow^{\bcB}\walM{\_}\mid \confGi$ and $\walM{\_}\mid\confG \rightarrow^{*}\walM{\_}\mid \confGii$ such that . Then for any minted token $(\tokT[0],\tokT[1])$, $\exchO[\confGi]{\tokT[0],\tokT[1]}\leq \exchO[\confGii]{\tokT[0],\tokT[1]}$.
% \end{lemma}
% \begin{proof}
% The lemma states that the prices of minted tokens after executing the 0-txpool game solution must be lower than minted token prices in any alternative state reachable from $\walM{\_}\mid\confG$ by the miner.

% We prove this lemma by contradiction: let us consider the user's wealth derived from its balance of \emph{atomic} and \emph{minted} tokens: in the \emph{0-txpool game}, the user does not perform any actions and thus, its token balance cannot change. If the token balance of the user remains constant, the only factor affecting an evolution in the user's wealth must be the price of minted tokens.

% Let us assume, that $\exchO[\confGi]{\tokT[0],\tokT[1]} > \exchO[\confGii]{\tokT[0],\tokT[1]}$ for any $(\tokT[0],\tokT[1])$, thereby contradicting the lemma: this implies there exists state $\walM{\_}\mid\confGii$ reachable by the miner, where the prices are lower than in $\walM{\_}\mid\confGi$  following the execution of the game solution $\bcB$: this is a contradiction, as the 0-txpool game solution must result in the minimized gain of the user and thus, minimized minted token prices.
% \end{proof}

% In order to produce a global optimum from a sequence of local optimizations in individual AMM pairs, the 0-txpool-swap game solution must ensure that the \emph{prices} of the AMM reserves are already minimized prior to the execution of the single AMM game. This is ensured by restricting the execution of 1-AMM-0-txpool games to pairs which only contain initial tokens (\jamesnote{step 1}) or minted tokens from pairs where the 1-AMM-0-txpool game has already been executed (\jamesnote{step 2}).

% \begin{theorem}
%   \label{th:0-txpool-swap-game}
%   Let \
%   $\confG = \walM{\tokBal} \mid \mmid_{i \in I} (\ammR[i,0]:\tokT[i,0],\ammR[i,1]:\tokT[i,1]) \mid \confG[w]$
%   be such that $\confG[w]$ only contains user wallets,
%   and let $\TxT = \emptymset$.
%   Then $\mev{\confG}{\TxT}$ and a solution $\bcB$ to the game is produced by the following algorithm:
%   \jamesnote{See algorithm 1. Deprecate in favor of greedy soln thm.}
% \end{theorem}

% \begin{algorithm}[t]
%   \begin{algorithmic}
%     \Function{Solve}{$\confG,\TxT$}
%     \Comment{$\confG = \mmid_{i \in I} (\ammR[i,0]:\tokT[i,0],\ammR[i,1]:\tokT[i,1]) \mid \confG[w]$}
%     \State $(\tokBal,\bcB) \gets (\emptyset,\emptyset,\emptyseq)$
%     \State $J \gets I$
%     \While {$J \neq \emptyset$}
%     \State choose $i \in J$
%       %     \State $\confG[i] \gets \confG[x] \text{ where } \confG \rightarrow^{\bcB} \confG[x]$
%     \If{$\swapGain{d}{\tokT[i,0],\tokT[i,1]}{\confG}{\tokBal} > 0$}
%     \State $\valV[0],\valV[1] \gets \swapVal[0]{d}{\tokT[i,0],\tokT[i,1]}{\confG}{}, \swapVal[1]{d}{\tokT[i,0],\tokT[i,1]}{\confG}{}$
%     \State $\tokBal \gets \tokBal + \valV[d]:\tokT[i,d]$ \jamesnote{notation}
%     \State $\bcB \gets \bcB :: (\actAmmSwap{\pmvM}{d}{\valV[0]}{\tokT[i,0]}{\valV[1]}{\tokT[i,1]})$
%     \EndIf
%     \State $J \gets J \setminus \setenum{i}$
%     \EndWhile
%     \State \Return $(\tokBal,\bcB)$
%     \EndFunction
%   \end{algorithmic}
%   \caption{Solution of the 0-txpool swap game \jamesnote{per greedy soln thm}}
%   \label{fig:0-txpool-swap-game}
% \end{algorithm}


\subsection{1-txpool game}
\label{sec:1txpool-game}

In this variant of the mining game,
we assume that the miner can perform actions on multiple AMMs,
and that $\TxT$ contains exactly one transaction.
Here, it is helpful to consider the wealth of $\pmvA$ as wealth components from both \emph{minted} and \emph{atomic} token balances:
\begin{equation}
  \label{eq:wealth-components}
  W_{\pmvA}(\confG) \; =
  \!\!\!
  \sum_{\tokT \in \dom(\tokBal)\cap\TokU[0]} \!\!\!\!\!
  \tokBal(\tokT)\cdot \exchO{\tokT}
  \;\;\; +
  \sum_{\tokT \in \dom(\tokBal) \cap \TokU[1]} \!\!\!\!\!
  \tokBal(\tokT) \cdot \exchO[\confG]{\tokT}
\end{equation}

In the 0-txpool game, the net worth of users is only affected by changes in the prices of minted tokens, since no user actions are performed which exchange units of tokens: thus, if for all users the net worth either stays constant or is reduced, the miner gain must be positive (\Cref{lma:wealth-conservation}).
Further, if the minted token prices are minimized, the miner's gain must be maximized.

In the 1-txpool game, only a single user will experience a change in its balance if the miner includes the user transaction in the solution. Further, atomic token prices are fixed whilst minted token prices are minimized by the miner, since they reduce the net worth of users holding such tokens, thereby implying a gain for the miner.

The strategy of the miner is to first consider whether to include the user action, and then to subsequently perform the canonical swap on all pairs, which can be interpreted as a 0-txpool game. Importantly, the following lemma states that the 0-txpool game played in two states, where one is reachable from the other, will always result in the same minted token prices.
\begin{lemma}
  \label{lma:minimized-prices}
  Let $\walM{\tokBal}\mid\confG[0]\rightarrow^{*}\walM{\_}\mid\confG[1]$, where $\confG[0] = \mmid_{i \in I} (\ammR[i,0]:\tokT[i,0],\ammR[i,1]:\tokT[i,1]) \mid \confG[w]$ be such that $\confG[w]$ only contains user wallets, and AMM reserves of all pairs $i\in I$ are non-zero in the execution. Let:
  \begin{equation}
    \walM{\tokBal[0]}\mid\confG[0] \xrightarrow{\bcB[0]}\walM{\_}\mid\confGi[0]
    \qquad
    \walM{\tokBal[1]}\mid\confG[1] \xrightarrow{\bcB[1]}\walM{\_}\mid\confGi[1]
  \end{equation}
  where $(\tokBal[0],\bcB[0])$ and $(\tokBal[1],\bcB[1])$ are
  solutions in $(\confG[0],\emptymset)$ and $(\confG[1],\emptymset)$,
  respectively.
  Then, $\exchO[{\confGi[0]}]{\tokT[i,0],\tokT[i,1]} = \exchO[{\confGi[1]}]{\tokT[i,0],\tokT[i,1]}$ for all $i\in I$.
\end{lemma}


A practical consequence of~\Cref{lma:minimized-prices} is that user actions
do not affect the price minimization performed by the miner to maximize its gain: the decision to include or drop a user transaction does not affect the minted token prices resulting from a subsequent 0-txpool game.
Thus, if including the user transaction increases the miner gain,
it will always be included in the 1-txpool game solution.

For a user $\ammSwapOp$ action, the exchanged value of atomic tokens determines whether it is profitable for the miner. The miner therefore executes the user swap, if the value of atomic tokens sent by the user is higher than value of atomic tokens received. In the subsequent state, the miner executes the 0-txpool game solution, thereby minimizing all minted token prices. The swapping user has its wealth reduced: both from the swap and the reduced price of minted tokens it holds. All other users have their weath reduced by the minimization of minted token prices. Thus, by \Cref{lma:wealth-conservation}, the miner must experience a positive gain. In some cases, maximizing the gain resulting from the user swap requires a front-run transaction by the miner.

A user $\ammDepositOp$ action does not affect the user's net worth during the execution step:
however, by \emph{increasing} the balance of the user's minted tokens,
any subsequent reduction of minted tokens caused by $\pmvM$
can increase the reduction \bartnote{??} of the user's net worth,
thereby motivating its inclusion.
%
By contrast, a user $\ammRedeemOp$ action is \emph{not} included in the solution of the 1-txpool game,
as a $\ammRedeemOp$ step does not change the net worth of the user and the prices of redeemed tokens cannot be negatively affected by subsequent miner actions.

We proceed by providing an overview of the 1-txpool game solutions by user action type, each followed by specific examples.
We conclude the section by formalizing auxiliary definitions and the general solution to the 1-txpool game in~\Cref{thm:1-txpool-game-soln}.

\mypar{User swap} The solution to the 1-txpool game solution includes the user swap action if it can be enabled such that (1) the user gain is minimized and (2) the user gain is negative. For $\actAmmSwap{\pmvA}{d}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}$ condition (1) holds if the user receives $\valV[1-d]:\tokT[1-d]$ in the swap execution and condition (2) holds if $\valV[1-d]\cdot\exchO{\tokT[1-1]}-\valV[d]\cdot\exchO{\tokT[d]} < 0$.
Here, it may be necessary for the miner to front-run the user swap action, in order to enable the user swap such that condition (1) holds. We denote this the \emph{swap front-run transaction} performed by the miner~\eqref{eq:canon-sf-swap}. Following the execution of the canonical swap front-run and user swap (if unprofitable for the user), the miner has minimized $\pmvM$'s wealth derived from its \emph{atomic} token balance~\eqref{eq:wealth-components}. In the subsequent state, no further user action is considered, such that the miner can only further reduce each users wealth by minimizing the price of minted tokens: this is equivalent to the 0-txpool game.

We now define the canonical swap front-run transaction.
For $\confG = (\ammR[0]:\tokT[0],\ammR[1]:\tokT[1]) \mid \cdots$ and $\txT = \actAmmSwap{\pmvA}{\swapDir[\pmvA]}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}$,
let the \keyterm{canonical swap front-run reserves} be
\begin{equation*}
  % \label{eq:canon-sf-reserves}
  \begin{split}
    \resSwap[{\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT)
    & = \frac{\abs{\sqrt{\valV[0]^2\cdot\valV[1]^2 + 4\cdot\valV[0]\cdot\valV[1]\cdot\ammR[0]\cdot\ammR[1]}\;}-\valV[0]\cdot\valV[1]}{2\cdot\valV[{{1-\swapDir[\pmvA]}}]}
    \\
    \resSwap[{1-\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT)
    & = \frac{\ammR[0]\cdot\ammR[1]}{\resSwap[{\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT)}
  \end{split}
\end{equation*}
These reserve values define a state $\confGi$ which is reachable from $\walM{\tokBal}\mid\confG$ with a \emph{canonical swap front-run transaction} by the miner.
\begin{equation}
  \label{eq:canon-sf-state}
  \confGi = (\resSwap[{\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT):\tokT[{\swapDir[\pmvA]}], \resSwap[{1-\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT) \mid \cdots
\end{equation}
Further, let the \keyterm{canonical swap front-run direction} be:
\begin{equation}
\label{eq:canon-sf-direction}
\swapDir[\pmvM] = \begin{cases} \swapDir[\pmvA] & \text{if } \resSwap[{\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT) > \ammR[{\swapDir[\pmvA]}] \\
  1-\swapDir[\pmvA] & \text{if } \resSwap[{1-\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT) > \ammR[{1-\swapDir[\pmvA]}] \end{cases}
\end{equation}
We define the \keyterm{canonical swap front-run values} as
\begin{equation*}
  % \label{eq:canon-sf-values}
\begin{split}
  \frontSwapVal[{{\swapDir[\pmvM]}}]{}{\tokT[0],\tokT[1],\confG}{\txT}{}
  & = \begin{cases} \resSwap[{\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT)-\ammR[{\swapDir[\pmvA]}] & \text{if } \swapDir[\pmvM] = \swapDir[\pmvA] \\
    \ammR[{\swapDir[\pmvA]}] - \resSwap[{\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT) &  \text{if } \swapDir[\pmvM] = 1-\swapDir[\pmvA] \end{cases}
  \\
  \frontSwapVal[{{1-\swapDir[\pmvM]}}]{}{\tokT[0],\tokT[1],\confG}{\txT}{}
  & = \begin{cases} \ammR[{1-\swapDir[\pmvM]}]-\resSwap[{1-\swapDir[\pmvM]}](\tokT[0],\tokT[1],\confG,\txT) & \text{if } \swapDir[\pmvM] = d \\
    \resSwap[{1-\swapDir[\pmvM]}](\tokT[0],\tokT[1],\confG,\txT)-\ammR[{1-\swapDir[\pmvM]}] &  \text{if } \swapDir[\pmvM] = 1-\swapDir[\pmvM] \end{cases}
\end{split}
\end{equation*}

\noindent
Finally, the \keyterm{canonical swap front-run transaction} is given by:
\begin{align}
  \label{eq:canon-sf-swap}
  & \frontSwapTx{\tokT[0],\tokT[1],\confG}{\txT}{}
  \\
  \nonumber
  & =
  \actAmmSwap
  {\pmvM}
  {\swapDir[\pmvM]}
  {\frontSwapVal[0]{}{\tokT[0],\tokT[1],\confG}{\txT}{}}{\tokT[0]}
  {\frontSwapVal[1]{}{\tokT[0],\tokT[1],\confG}{\txT}{}}{\tokT[1]}
\end{align}


\begin{figure}[t]
  \small
  \scalebox{0.95}{\parbox{\textwidth}{%
      \begin{align}
        \nonumber
        & \walM{35:\tokT[1]} \mid
          \walA{40:\tokT[0]} \mid
          (100:\tokT[0],100:\tokT[1]) \mid \cdots
        \\
        \nonumber
        % \xrightarrow{\actAmmSwapR{\pmvM}{11.2}{\tokT[0]}{12.7}{\tokT[1]}} \;
        \xrightarrow{\frontSwapTx{\tokT[0],\tokT[1],\confG}{\txT}{}}
        & \walM{11.2:\tokT[0],22.3:\tokT[1]} \mid
          (88.8:\tokT[0],112.7:\tokT[1]) \mid \cdots
        \\
        \nonumber
        \xrightarrow{\txT = \actAmmSwapL{\pmvA}{40}{\tokT[0]}{35}{\tokT[1]}} \;
        & \walA{0:\tokT[0],35:\tokT[1]} \mid
          (128.8:\tokT[0],77.7:\tokT[1]) \mid \cdots
        \\
        \nonumber
        % \xrightarrow{\actAmmSwapR{\pmvM}{28.7}{\tokT[0]}{22.3}{\tokT[1]}} \;
        \xrightarrow{\swapTx{\tokT[0],\tokT[1]}{\confGii}{}}
        & \walM{40:\tokT[0],0:\tokT[1]} \mid
          (100:\tokT[0],100:\tokT[1]) \mid \cdots
      \end{align}}}
  \vspace{-10pt}
  \caption{1-txpool game solution with a user swap.}
  \label{fig:swap-front-run}
\end{figure}


\begin{example}
  \label{ex:1txpool-game-sf}
  Recall the example in \Cref{sec:intro} and in \Cref{sec:miner:sandwich},
  where $\pmvA$ emits a transaction $\txT = \actAmmSwapL{\pmvA}{40}{\tokT[0]}{35}{\tokT[1]}$ in state $\confG = (100:\tokT[0],100:\tokT[1]) \mid\confG[w]$, where $\confG[w]$ only contains user wallets, $ \walA{40:\tokT[0]} \in \confG[w]$ and $\exchO{\tokT[0]} = \exchO{\tokT[1]} = 1,000$.
  The execution of the game solution $(\tokBal,\bcB)$ is shown in~\Cref{fig:swap-front-run}, which recasts \Cref{fig:sandwich} with the notation of this section. The user action must be included in the game solution since $35\cdot\exchO{\tokT[1]}-40\cdot\exchO{\tokT[1]} = 35,000-40,000 = -5,000$ is negative.
  In order to realize this gain, a canonical swap front-run transaction is needed: we compute the \emph{canonical swap front-run reserves}
  for the 1-txpool game $(\confG,\msetenum{\txT})$:
  \begin{align*}
    \resSwap[0](\txT,\confG)
    & = \frac{\sqrt{40^2\cdot35^2 +4\cdot40\cdot35 \cdot100^2}-40\cdot35}{2\cdot35} \approx 88.8
    \\
    \resSwap[1](\txT,\confG)
    & = \frac{100^2}{89} \approx 112.7
  \end{align*}
  Since $\resSwap[i](\txT,\confG) \not= 100$ for $i\in\setenum{0,1}$
  and thus differs from the reserves in the initial game state,
  the miner must first fire a user front-run transaction
  $\walM{\tokBal} \mid \confG \myxrightarrow{\frontSwapTx{\txT}{\confG}{}} \walM{\tokBali} \mid \confGi$ such that
  \begin{equation*}
    \confGi
    =
    \walA{40:\tokT[0]}\mid(\resSwap[{\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT):\tokT[{\swapDir[\pmvA]}], \resSwap[{1-\swapDir[\pmvA]}](\tokT[0],\tokT[1],\confG,\txT) \mid \cdots
  \end{equation*}

  By definition, firing $\txT$ in $\walM{\tokBali} \mid \confGi$
  results in the minimized user step gain $\gain{\pmvA}{\walM{\tokBali}\mid\confGi,\txT} = -5,000$.
  Since $\resSwap[1](\tokT[0],\tokT[1],\confG,\txT) > \ammR[1]$,
  the direction~\eqref{eq:canon-sf-direction} of the front-running swap is $\swapDir[\pmvM] = 1$.
  Thus, we can compute the \emph{canonical swap front-run values}
  and \emph{canonical swap front-run transaction} as:
  \begin{align*}
    \frontSwapVal[0]{}{\tokT[0],\tokT[1],\confG}{\txT}{}
    & = 100 - 88.8 \approx 11.2
    \\
    \frontSwapVal[1]{}{\tokT[0],\tokT[1],\confG}{\txT}{}
    & = 112.7 - 100 \approx 12.7
    \\
    \frontSwapTx{\tokT[0],\tokT[1],\confG}{\txT}{}
    & =
    \actAmmSwap
    {\pmvM}
    {1}
    {11.2}{\tokT[0]}
    {12.7}{\tokT[1]}
  \end{align*}
  Here, $\pmvM$ can perform $ \frontSwapTx{\tokT[0],\tokT[1],\confG}{\txT}{}$
  with $\tokBal(\tokT[1]) \geq 12.7$.
  After firing the canonical swap front-run and the user swap,
  we derive the 0-txpool solution in $\confGii = (128.8:\tokT[0],77.7:\tokT[1]) \mid \cdots$, shown in~\Cref{fig:swap-front-run}.
  For $\confGii$, the canonical swap values and transaction are:
  \begin{align*}
    \swapVal{1}{\tokT[0],\tokT[1]}{\confGii}{}
    & = \sqrt{\tfrac{1}{1} \cdot 128.8 \cdot 77.7} - 77.7 \approx 22.3
    \\
    \swapVal{0}{\tokT[0],\tokT[1]}{\confGii}{}
    & = \frac
      {128.8 \cdot 22.3}
      {77.7 + 22.3} \approx 28.7
  \end{align*}
  \[
  \swapTx{\tokT[0],\tokT[1]}{\confGii}{} =
  \actAmmSwap
  {\pmvM}
  {1}
  {28.7}{\tokT[0]}
  {22.3}{\tokT[1]}
  \]
  Considering the entire run from $\walM{\tokBal}\mid\confG$,
  we determine $\pmvM$'s gain as
  $\gain{\pmvM}{\walM{\tokBal}\mid\confG,\bcB}= (11.2 - 12.7)\cdot 1,000 + (28.7-22.3) \cdot 1,000 \approx 5,000$, which is the loss of the user $\pmvA$.
  We can construct the miner balance $\tokBal$ greedily as the sum of all input amounts in the solution trace.
  Thus, our solution to the 1-txpool game $(\confG,\msetenum{\txT})$ is:
  \[
\tokBal =
% \setenum{\tokT[1] :12.7+22.3} =
\setenum{\tokT[1]:35}
\qquad
\bcB = \frontSwapTx{\tokT[0],\tokT[1],\confG}{\txT}{} \ \txT \ \swapTx{\tokT[0],\tokT[1]}{\confGii}{}
\tag*{$\qed$}
\]
\end{example}

% In the case of $\TxT = \setenum{\actAmmSwap{\pmvA}{\swapDir[\pmvA]}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}}$, let $\swapDir[\pmvA]$ denote the swap direction by the user. As defined in $\nrule{[Swap]}$, $\valV[1-{\swapDir[\pmvA]}]$ indicates a \emph{minimum} amount of $\tokT[1-{\swapDir[\pmvA]}]$ the user must receive when performing swap: if $\valV[{{1-\swapDir[\pmvA]}}]\cdot \exchO{\tokT[{1-\swapDir[\pmvA]}]} -\valV[{{\swapDir[\pmvA]}}]\cdot\exchO{\tokT[{\swapDir[\pmvA]}]}$ is negative for the user, the rational miner will include it in the game solution. Further, the miner must ascertain whether a \emph{canonical swap front-run} action is necessary in order to reach a state in which the user swap action results in the aforementioned \emph{minimal} gain for the user.

% In the subsequent~\Cref{thm:1-txpool-game-soln}, we show that the trace $\bcB$ in our solution $(\tokBal,\bcB)$ to the 1-txpool game with $(\TxT = \setenum{\pmvA:\ammSwapOp},\confG)$ begins with a canonical swap front-run by the miner (if defined), followed by $\pmvA:\ammSwapOp$ and then the 0-txpool game solution to $(\emptyset, \confGi)$, where $\walM{\tokBal}\mid\confG \rightarrow^{\pmvA:\ammSwapOp}\walM{\tokBali}\mid\confGi$. The following example is intended to provide an illustration of this result.

\mypar{User deposit} The solution to the 1-txpool game will include a user deposit action if it deposits funds in the AMM in a state,
from which the minted token price can further be reduced by miner actions.
For a deposit $\actAmmDeposit{\pmvA}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}$ in the 1-txpool game $(\confG,\msetenum{\txT})$, this is the case when
\[
  \frac{\valV[0]}{\valV[1]}
  \; \not= \;
  \frac{\exchO{\tokT[1]}}{\exchO{\tokT[0]}}
\]
holds, since in a reachable state $\confG= (\ammR[0]:\tokT[0],\ammR[1]:\tokT[1])\mid \cdots$ where the deposit $\txT$ is enabled,
\begin{align*}
  \frac{\valV[0]}{\valV[1]}
  \; = \;
  \frac{\ammR[0]}{\ammR[1]}
  \; \not= \;
  \frac{\exchO{\tokT[1]}}{\exchO{\tokT[0]}}
\end{align*}
and the values of the pair reserves are such, that a canonical swap is defined (\Cref{sec:1amm-0txpool-game}).
Thus, although the deposit action step maintains the net wealth of $\pmvA$, the price of minted tokens $(\tokT[0],\tokT[1])$ received by the user in the deposit can subsequently be reduced by a canonical swap performed by the miner.

Here too, it may be necessary for the miner to front-run the user deposit in order enable its execution.
We provide auxiliary definitions to formalize the \emph{canonical deposit front-run transaction}.

For $\confG= (\ammR[0]:\tokT[0],\ammR[1]:\tokT[1])\mid \cdots$ and $\txT = \actAmmDeposit{\pmvA}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}$, let us denote the \keyterm{canonical deposit front-run reserves} as
\begin{equation}
  \label{eq:canon-df-reserves}
  \begin{array}{c}
    \resDeposit[0](\tokT[0],\tokT[1],\confG,\txT)
    = \left|\sqrt{\frac{\valV[0]}{\valV[1]} \cdot \ammR[0] \cdot \ammR[1]}\:\right|
    \\[9pt]
    \resDeposit[1](\tokT[0],\tokT[1],\confG,\txT)
    = \left|\sqrt{\frac{\valV[1]}{\valV[0]} \cdot \ammR[0] \cdot \ammR[1]}\:\right|
  \end{array}
\end{equation}
which satisfy:
\[
  \frac{\resDeposit[0](\tokT[0],\tokT[1],\confG,\txT)}{\resDeposit[1](\tokT[0],\tokT[1],\confG,\txT)} = \frac{\valV[0]}{\valV[1]}
\]
Further, we define the \keyterm{canonical deposit front-run values} as:
\begin{equation}
\label{eq:canon-df-values}
\begin{split}
  \frontDepVal[{{\swapDir[\pmvM]}}]{}{\tokT[0],\tokT[1],\confG}{\txT}{}
  & = \resDeposit[{\swapDir[\pmvM]}](\tokT[0],\tokT[1],\confG,\txT) - \ammR[{\swapDir[\pmvM]}]
  \\
  \frontDepVal[{{1-\swapDir[\pmvM]}}]{}{\tokT[0],\tokT[1],\confG}{\txT}{}
  & = \ammR[{1-\swapDir[\pmvM]}] - \resDeposit[{1-\swapDir[\pmvM]}](\tokT[0],\tokT[1],\confG,\txT)
\end{split}
\end{equation}
\noindent
if a swap direction $\swapDir[\pmvM]$ satisfies both:
\[
\frontDepVal[{{\swapDir[\pmvM]}}]{}{\tokT[0],\tokT[1],\confG}{\txT}{} > 0
\qquad
\frontDepVal[{{1-\swapDir[\pmvM]}}]{}{\tokT[0],\tokT[1],\confG}{\txT}{} > 0
\]
then we define the \keyterm{canonical deposit front-run transaction} as:
\begin{align}
  \label{eq:canon-df-transaction}
  & \frontDepTx{\tokT[0],\tokT[1],\confG}{\txT}{}
  \\
  \nonumber
  & = \actAmmSwap
    {\pmvM}{{\swapDir[\pmvM]}}
    {\frontDepVal[0]{}{\tokT[0],\tokT[1],\confG}{\txT}{}}{\tokT[0]}
    {\frontDepVal[1]{}{\tokT[0],\tokT[1],\confG}{\txT}{}}{\tokT[1]}
\end{align}

The following example show how the miner can front-run a user deposit with a \emph{canonical deposit front-run transaction}.

\begin{example}
  \label{ex:1txpool-game-df}
  Let $\txT = \actAmmDeposit{\pmvA}{60}{\tokT[0]}{40}{\tokT[1]}$,
  and let $\confG = (50:\tokT[0],50:\tokT[1]) \mid \confG[w]$,
  where $\confG[w]$ only contains user wallets,
  $\walA{60:\tokT[0],40:\tokT[1]} \in \confG[w]$,
  and $\exchO{\tokT[0]} = \exchO{\tokT[1]} = 1$.
  The execution of the solution is shown in~\Cref{fig:deposit-front-run}.
  By rule $\nrule{[Dep]}$, $\txT$ cannot be fired in $\confG$, since the deposit ratio $60/40$ does not equal the reserve ratio $50/50$ of the $(\ammR[0],\ammR[1])$ pair: however, this also implies that the miner can profit from executing the user deposit in the game solution.

  In order to execute $\txT$, $\pmvM$ must produce a front-running transaction.
  We first compute the \emph{canonical deposit front-run} pair reserves:
  \begin{align*}
    \nonumber
    \resDeposit[0](\tokT[0],\tokT[1],\confG,\txT)
    & = \left|\sqrt{\frac{60}{40} \cdot 50^2}\:\right| \approx 61.2
    \\
    \resDeposit[1](\tokT[0],\tokT[1],\confG,\txT)
    & = \frac{40 \cdot 61.2}{60} \approx 40.8
  \end{align*}
  This gives the following \emph{canonical deposit front-run} values:
  \begin{align*}
    \frontDepVal[0]{}{\tokT[0],\tokT[1],\confG}{\txT}{}
    & = 61.2-50 \approx 11.2
    \\
    \frontDepVal[1]{}{\tokT[0],\tokT[1],\confG}{\txT}{}
    & = 50-40.8 \approx 9.2
  \end{align*}

  \noindent
  and the \emph{canonical deposit front-run transaction} is:
  \[
  \frontDepTx{\tokT[0],\tokT[1],\confG}{\txT}{}
  =
  \actAmmSwap
  {\pmvM}
  {0}
  {11.2}{\tokT[0]}
  {9.2}{\tokT[1]}
  \]

  \begin{figure}[t]
    \small
    \scalebox{0.95}{\parbox{\textwidth}{% d
      \begin{align}
        \nonumber
        & \walM{11.2:\tokT[0],18.2:\tokT[1]} \mid
          \walA{60:\tokT[0],40:\tokT[1]} \mid
          (50:\tokT[0],50:\tokT[1]) \mid \cdots
        \\
        \nonumber
        \xrightarrow{\frontDepTx{\tokT[0],\tokT[1],\confG}{\txT}{}} \;
        & \walM{0:\tokT[0],27.4:\tokT[1]} \mid
          (61.2:\tokT[0],40.8:\tokT[1]) \mid \cdots
        \\
        \nonumber
        \xrightarrow{\txT=\actAmmDeposit{\pmvA}{60}{\tokT[0]}{40}{\tokT[1]}} \;
        & \walA{0:\tokT[0],0:\tokT[1],49.0:(\tokT[0],\tokT[1])} \mid
          (121.2:\tokT[0],80.8:\tokT[1]) \mid \cdots
        \\
        \nonumber
        \xrightarrow{\swapTx{\tokT[0],\tokT[1]}{\confGii}{}} \;
        & \walM{22.2:\tokT[0],9.2:\tokT[1]} \mid
          (99.0:\tokT[0],99.0:\tokT[1]) \mid \cdots
      \end{align}}}
    \vspace{-10pt}
    \caption{1-txpool game solution with a user deposit.}
    \label{fig:deposit-front-run}
  \end{figure}

  Following the canonical deposit front-run by the miner, the user's deposit $\txT$ can now be executed. For $\txT$ in~\Cref{fig:deposit-front-run}, note that we assume that the supply of $(\tokT[0],\tokT[1])$ is $50$
  in the initial state $\confG$.
  Thus, the minted amount $\pmvA$ receives for the deposit is:
  \[
  \valV
  \; = \;
  \frac{\valV[0]}{\ammR[0]}\cdot \supply{\tokT[0],\tokT[1]}(\confG)
  \; = \;
  \frac{60}{61.2} \cdot 50
  \; \approx \;
  49
  \]
  To determine the required miner balance, we simply aggregate the transaction \emph{input} amounts from all miner actions. Thus, a solution to our 1-txpool game with a user deposit is given by $(\tokBal,\bcB)$ where:
  \begin{align*}
    \tokBal &= \setenum{11.2:\tokT[0],18.1:\tokT[1]}
    \qquad
    \bcB = \frontDepTx{\tokT[0],\tokT[1]\confG}{\txT}{} \ \txT \ \swapTx{\tokT[0],\tokT[1]}{\confGii}{}
  \end{align*}
  and $\confGii$ is determined by:
  \[
  \walM{\tokBal} \mid \confG
  \; \xrightarrow{\frontDepTx{\tokT[0],\tokT[1],\confG}{\txT}{}} \walM{\tokBali} \mid \confGi \;
  \; \xrightarrow{\txT} \;
  \walM{\tokBalii} \mid \confGii
  \]
  Finally, we compute the gain of $\pmvA$ and of $\pmvM$ as follows:
  \begin{align*}
    \gain{\pmvA}{\confG,\bcB}
    & =
      \Big( \frac{49.0}{99.0}\cdot99.9 - 60 \Big) + \Big( \frac{49.0}{99.0}\cdot99.9 - 40 \Big) = -2.0
    \\
    \gain{\pmvM}{\confG,\bcB}
    & = - \gain{\pmvA}{\confG,\bcB} = 2
      \tag*{$\qed$}
  \end{align*}
\end{example}


\mypar{User redeem}

Unlike user deposits, user redeems will \emph{reduce} the MEV for the miner.
% this happens when $\pmvA$ redeems minted tokens $(\tokT[0],\tokT[1])$.
If a redeem of $(\tokT[0],\tokT[1])$ occurs in a state where the price of $(\tokT[0],\tokT[1])$ is not minimized, $\pmvA$ will experience a \emph{reduced} depreciation of her minted tokens.

% \jamesnote{TODO: reconsider if 1-txpool 1-amm game.}
% \begin{lemma}
%   \label{lma:no-rdm-frontrun}
%   Let $\confG = \mmid_{i \in I} (\ammR[i,0]:\tokT[i,0],\ammR[i,1]:\tokT[i,1]) \mid \confG[w]$,
%   where $\confG[w]$ contains $\tokBal[\pmvA]$,
%   and $\TxT = \setenum{\actAmmRedeem{\pmvA}{\valV:(\tokT[j,0],\tokT[j,1])}}$ such that $j\in I$. Then a 0-txpool game solution in $\confG$ is also a solution to the 1-txpool game in $\confG$.
% \end{lemma}

\begin{example}
  \label{ex:1txpool-game-redeem}
  Let $\txT = \actAmmRedeem{\pmvA}{20:(\tokT[0],\tokT[1])}$ and $\confG = (100:\tokT[0],100:\tokT[1])  \mid \confG[w]$ where $\confG[w]$ contains only wallets, $\walA{20:(\tokT[0],\tokT[1])} \in \confG[w]$ and $\exchO{\tokT[0]} = 1.3$ and $\exchO{\tokT[1]} = 1$.
  We show an execution of game solution,
  where $\bcB = \swapTx{\tokT[0],\tokT[1]}{\confG}{} = \actAmmSwapR{\pmvM}{12.3}{\tokT[0]}{14.0}{\tokT[1]}$:
  \\
  {\small
  \scalebox{0.95}{\parbox{\textwidth}{%
      \begin{align}
        \nonumber
        & \walA{20:(\tokT[0],\tokT[1])} \mid
          \walM{14.0:\tokT[1]} \mid (100:\tokT[0],100:\tokT[1])
        \\
        \nonumber
        \xrightarrow{\actAmmSwapR{\pmvM}{12.3}{\tokT[0]}{14.0}{\tokT[1]}} \;
        & \walA{\cdots} \mid
          \walM{12.3:\tokT[0],0:\tokT[1]} \mid (87.7:\tokT[0],114:\tokT[1])
      \end{align}}}
  }%
  \\
  where the miner gain $\gain{\pmvM}{\confG,\bcB} = 12.3\cdot1.3 - 14.0\cdot 1 \approx 2.0$.

  We show a non-optimal, alternative trace,
  which \emph{includes} $\pmvA$'s redeem,
  to illustate how $\pmvM$'s gain is \emph{reduced} by $\pmvA$'s redeem.
  \\
  {\small
  \scalebox{0.95}{\parbox{\textwidth}{%
      \begin{align}
        \nonumber
        & \walA{20:(\tokT[0],\tokT[1])} \mid
          \walM{11.2:\tokT[1]} \mid (100:\tokT[0],100:\tokT[1]) \mid \cdots
        \\
        \nonumber
        \xrightarrow{\actAmmRedeem{\pmvA}{20:(\tokT[0],\tokT[1])}} \;
        & \walA{20:\tokT[0],20:\tokT[1]} \mid
          (80:\tokT[0],80:\tokT[1]) \mid \cdots
        \\
        \nonumber
        \xrightarrow{\actAmmSwapR{\pmvM}{9.8}{\tokT[0]}{11.2}{\tokT[1]}} \;
        & \walA{\cdots} \mid
          \walM{9.8:\tokT[0],0:\tokT[1]} \mid
          (70.2:\tokT[0],91.2:\tokT[1]) \mid \cdots
      \end{align}}}}
  \\
  Here the miner gain is $\gain{\pmvM}{\confG,\bcB} = 9.8\cdot1.3 - 11.2\cdot 1 \approx 1.6$. Note that reduction in gain results from the reduced swap amounts performed in the 0-txpool game following the user redeem: this is due to the deposit reduction resuling from the user's redeem.
  \qed
\end{example}



\mypar{Solution to the 1-txpool game}

Having provided canonical definitions for action-specific scenarios of the 1-txpool game solution, we can now state the general 1-txpool game solution.

\begin{theorem}
  \label{thm:1-txpool-game-soln}
  Let $\confG = \mmid_{i \in I} (\ammR[i,0]:\tokT[i,0],\ammR[i,1]:\tokT[i,1]) \mid \confG[w]$,
  where $\confG[w]$ contains only wallets, including $\walA{{\tokBal[\pmvA]}}$,
  and let $\TxT = \msetenum{\txT}$.
  Then:
  \mypar{Case 1}
  If $\:\txT = \actAmmSwap{\pmvA}{\swapDir[\pmvA]}{\valV[0]}{\tokT[j,0]}{\valV[1]}{\tokT[j,1]}$, $j\in I$ and
  \[
  \tokBal[\pmvA] \tokT[j,{\swapDir[\pmvA]}] \geq \valV[j,{\swapDir[\pmvA]}]
  \qquad
  \valV[{{\swapDir[\pmvA]}}] \cdot \exchO{\tokT[j,{\swapDir[\pmvA]}]} > \valV[1-{\swapDir[\pmvA]}] \cdot \exchO{\tokT[j,1-{\swapDir[\pmvA]}]}
  \]
  hold true, let
  \begin{equation}
    \nonumber
    \begin{array}{l}
      \begin{split}
        \tokBal &= \setenum{\frontSwapVal[{{\swapDir[\pmvM]}}]{}{\tokT[0],\tokT[1],\confG}{\txT}{} : \tokT[j,{\swapDir[\pmvM]}]}
        \\
        \bcB &= \begin{cases}
          \frontSwapTx{\tokT[0],\tokT[1],\confG}{\txT}{} \ \txT & \text{if }\:\frontSwapTx{\tokT[0],\tokT[1],\confG}{\txT}{} \text{ is defined}\\
          \txT & \text{otherwise}
        \end{cases}
      \end{split}
      \\
      \walM{\tokBal} \mid \confG \xrightarrow{\bcB} \walM{\_} \mid \confGi
      \\[5pt]
      (\tokBali, \bcBi) \quad \text{be a solution to the game in $(\confGi,\emptymset)$}
    \end{array}
  \end{equation}
  Then, $(\tokBal + \tokBali,\bcB \bcBi)$ is a solution to the game
  in $(\confG,\TxT)$.
  \mypar{Case 2} If $\;\txT = \actAmmDeposit{\pmvA}{\valV[0]}{\tokT[j,0]}{\valV[1]}{\tokT[j,1]}$, $j\in I$ and
  \[
  (\tokBal[\pmvA] \tokT[j,0],\tokBal[\pmvA] \tokT[j,1]) \geq (\valV[0],\valV[1])
  \qquad
  \frac{\valV[0]}{\valV[1]}
  \; \not= \;
  \frac{\exchO{\tokT[j,1]}}{\exchO{\tokT[j,0]}}
  \]
  hold true, let
  \begin{equation}
    \nonumber
    \begin{array}{l}
      \begin{split}
        \tokBal &= \setenum{\frontDepVal[{{\swapDir[\pmvM]}}]{}{\tokT[0],\tokT[1],\confG}{\txT}{} : \tokT[j,{\swapDir[\pmvM]}]}
        \\
        \bcB &= \begin{cases}
          \frontDepTx{\tokT[0],\tokT[1],\confG}{\txT}{} \ \txT & \text{if }\:\frontDepTx{\tokT[0],\tokT[1],\confG}{\txT}{} \text{ is defined}\\
          \txT & \text{otherwise}
        \end{cases}
      \end{split}
      \\
      \walM{\tokBal} \mid \confG \xrightarrow{\bcB} \walM{\_} \mid \confGi
      \\[5pt]
      (\tokBali, \bcBi) \quad \text{be a solution to the game in $(\confGi,\emptymset)$}
    \end{array}
  \end{equation}
  Then, $(\tokBal + \tokBali,\bcB \bcBi)$ is a solution to the game
  in $(\confG,\TxT)$.
  % \bartnote{I have introduced $\ammR[0],\ammR[1]$ to avoid using $res^L$}
  % \begin{equation}
  %   \nonumber
  %   \begin{array}{c}
  %     \gain[{\walM{\tokBal} \mid \confG}]{\pmvM}{\bcB}
  %     - \gain[{\walM{\tokBali} \mid \confGi}]{\pmvM}{\bcBi}
  %     \\[5pt] =
  %     \big(
  %     \valVi[{{1-\swapDiri[\pmvM]}}] \ \exchO{\tokT[{j,1-\swapDiri[\pmvM]}]}
  %     -
  %     \valVi[{{\swapDiri[\pmvM]}}] \ \exchO{\tokT[j,{{\swapDiri[\pmvM]}}]}
  %     \big)
  %     %
  %     \cdot
  %     \frac{\valV[0]}
  %     {\ammR[0]} > 0
  %     \\[7pt]
  %     \text{where}\quad
  %     \swapTx[{\swapDiri[\pmvM]}]{\tokT[j,0],\tokT[j,1]}{\confGi}{}
  %     \; = \;
  %     \actAmmSwap{\pmvM}{\swapDiri[\pmvM]}{\valVi[0]}{\tokT[j,0]}{\valVi[1]}{\tokT[j,1]}
  %   \end{array}
  % \end{equation}
  % Otherwise case.
  \mypar{Case 3}
  Otherwise, a solution of the 0-tx pool game in $(\confG,\emptymset)$ is a solution to the 1-txpool game in $(\confG,\TxT)$.
\end{theorem}



\subsection{The general game}
\label{sec:ntxpool-game}

% \bartnote{we do not construct a solution to the general version of the game: the greedy strategy may fail, because the order of transactions may affect which of $\pmvA$'s transactions can be enabled. It may also happen that the optimal solution allows $\pmvA$ to perform profitable transactions! These transactions may be needed to enable other transactions by $\pmvA$!!}

% \jamesnote{The N-txpool game can be solved greedily, by repeating the 1-txpool game, but it may not result in the soln with the fewest steps. Alternatively, we break the 1-txpool game into part 1 and 2(0-txpool game tx), and perform part 1 greedily for all txs, before concluding with part 2. This may result in fewer steps, but steps can be optimized further by pair order.}
% \albertonote{I would not mention the number of steps / block size here. Give the current status of the paper this ``dimension'' of the game should go into a discussion in the conclusion (e.g. as future work). }
% \jamesnote{we provide a partial solution to the n-txpool game.}

We construct a solution for the general game in $(\confG,\TxT)$,
by greedily composing 1-txpool game solutions for each action in $\TxT$.
Because the solution is constructed by evaluating each $\txT \in \TxT$ greedily, we must ensure that each user has a sufficient balance of atomic tokens to enable all its transactions in $\TxT$ in any order: we define the \emph{minimum input balance} in the general game $(\confG,\TxT)$ for $\pmvA$ as:
\begin{align*}
  \txInAmt{\pmvA,\TxT} &= \begin{cases}
    \txInAmt{\pmvA,\txT} + \txInAmt{\pmvA,\TxTi}
    & \text{if }
      \TxTi = \TxT \msetminus \msetenum{\txT} \not= \emptymset \\
    \txInAmt{\pmvA,\txT} & \text{if }\TxT = \msetenum{\txT}
  \end{cases}
  \\[5pt]
  \txInAmt{\pmvA,\txT} &= \begin{cases}
    \setenum{\valV[d]:\tokT[d]} & \txT = \actAmmSwap{\pmvA}{d}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]} \\
    \setenum{\valV[0]:\tokT[0],\valV[1]:\tokT[1]} & \txT = \actAmmDeposit{\pmvA}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]} \\
    \setenum{} & \txT = \actAmmRedeem{\pmvA}{\valV:(\tokT[0],\tokT[1])}
  \end{cases}
\end{align*}

A user must have a balance greater than its minimum input balance for its transactions to be considered in the general game.
Such minimum balance is defined inductively by only aggregating token amounts transferred away from the user in its transactions.
For redeems, no input token amounts are accounted for, as user redeem actions are not part of the 1-txpool and n-txpool solutions.

Notably, this constraint results in a less general solution for the general game: still, we believe it is not unrealistic: users are likely to only broadcast transactions to the network, such that their token balance is sufficient to enable all pending transactions in any order.

\begin{theorem}
  \label{thm:n-txpool-soln}
  Let $\confG = \mmid_{i \in I} (\ammR[i,0]:\tokT[i,0],\ammR[i,1]:\tokT[i,1]) \mid \confG[w]$,
  where $\confG[w]$ contains user wallets only,
  and let $\TxT$ be a set of user transactions. Furthermore, for all $\pmvA$ such that $\walA{{\tokBal[\pmvA]}} \in \confG[w]$, $\tokBal[\pmvA]\sqsupseteq \txInAmt{\pmvA,\TxT}$.

  \mypar{case 1} If $\TxT$ is empty, the solution to the n-txpool game is the 0-txpool game solution to $(\confG,\emptymset)$.

  \mypar{case 2} Otherwise, let $\TxT = \msetenum{\txT} \msetcup \TxTi$ and $(\tokBal,\bcB)$  be the 1-txpool game solution in $(\confG,\msetenum{\txT})$.
  Furthermore, let $\walM{\tokBal}\mid\confG \myxrightarrow{\bcB} \walM{\_}\mid\confGi$ and $(\tokBali,\bcBi)$ be the n-txpool game solution to $(\confGi,\TxTi)$.
Then the game solution to $(\confG,\TxT)$ is $(\tokBal+\tokBali,\bcB\bcBi)$.
\end{theorem}

Here the solution is defined inductively: individual 1-txpool game solutions are aggregated for one user transaction at a time in any order.
The minimum user input balance constraint ensures that each user balance enables its transactions in any sequence.
The main proof idea is that each user transaction does not impact the miner gain contribution of any other transaction in the game: it is easily shown that the effect of each transaction on the user's token balance does not depend on the order of their execution.
Further, \Cref{lma:minimized-prices} states that the minted token prices will always be equal after the 0-txpool game is played.
Therefore, both token balance and token prices do not depend on the transaction order and can be optimized for maximimum miner gain in a greedy fashion.

% Due to conservation of wealth, it is helpful to first consider the maximum possible loss experienced by users, since this loss may be inferred as a gain for the miner. \albertonote{Why inferred? Is the loss of the users not precisely the gain of the miners?}We first consider the potential loss a holder of minted tokens, if arbitrage is performed on the related AMM pair, such that no further arbitrage opportunity remains.

% \jamesnote{AMM pairs contain initial tokens only, $\fee = 1$, miner holds no minted tokens.}

% \jamesnote{If $\fee \neq 1$, then this does not hold in all cases, since the minted token price will be positively affected by fee accrual.}

% \bartnote{extracted from statement: in $\confGi$ the funds ratio for all AMM pairs is equal to the inverse of the respective token price ratio}


% \jamesnote{lma:max-token-depreciation moved to 4.3.}

% We define the \emph{extractable value} from a token pair $(\_:\tokT[0],\_:\tokT[1]) \in \confG$ as
% \begin{equation}
%   \begin{array}{c}
%     \mathit{ext}^{\confG}(\tokT[0],\tokT[1]) = \big(\exchO[\confGi]{\tokT[0],\tokT[1]} - \exchO[\confG]{\tokT[0],\tokT[1]} \big)
%     \cdot \supply{(\tokT[0],\tokT[1])}(\confG)
%     \\[3pt]
%     \text{ where } \confG \myxrightarrow{\ammSwapOp} \confGi
%     \\[3pt]
%     \ammRi[1]/\ammRi[0] = \exchO{\tokT[0]} / \exchO{\tokT[1]}
%     \quad
%     (\ammRi[0]:\tokT[0],\ammRi[1]:\tokT[1]) \in \confGi
%   \end{array}
% \end{equation}

% \jamesnote{WIP: how to define this to include nested tokens.}

% \bartnote{I have moved here this definition, because is does not seem to be used before}
% We define the gain of $\pmvA$ upon $\bcB$
% (without considering the initial state $\confG$) as
% the collection of all gains, for all possible initial $\confG$:
% \bartnote{$\confG$ reachable??}
% \[
% \gain{\pmvA}{\bcB}
% \; = \;
% \textstyle
% \bigcup_{\confG} \; \gain[\confG]{\pmvA}{\bcB}
% \]

% Next, we observe that certain user swap transactions can be executed such that the gain resulting from the execution step is minimized for the user.

% \begin{lemma}[Minimized user gain]
%   \label{lma:min-gain}
%   Let $\confG \xrightarrow{\txT} \confGi$,
%   with
%   $\txT = \pmvA:\ammSwapLOp(\valV[0]:\tokT[0],\valV[1]:\tokT[1])$. If $\tokBali[\pmvA]\tokT[1] - \tokBal[\pmvA]\tokT[1] = \valV[1]$, then $\gain[\confG]{\pmvA}{\txT} = min(\gain{\pmvA}{\txT})$.
% \end{lemma}

% Similarly for $\ammSwapROp$.
% We write $\txT_{\pmvA}$ minimizes user gain in $\confG$ if
% $\gain[\confG]{\pmvA}{\txT[\pmvM]} = min(\gain{\pmvA}{\txT[\pmvA]})$.
% If $min(G_{\pmvA}(\txT_{\pmvA})) \leq 0$, we write that a transaction is \emph{unprofitable} or \emph{strictly} unprofitable if the strict inequality holds. Due to wealth conservation, the execution of an unprofitable transaction can be interpreted as a positive gain or \emph{extractable value} for other actors, such as the miner. We define the extractable value for a transaction $\txT[\pmvA]$ as
% \[
% \small
% \mathit{ext}(\txT[\pmvA]) = \begin{cases}
%   - \mathit{min}(\gain{\pmvA}{\txT[\pmvA]})
%   & \mathit{min}(\gain{\pmvA}{\txT[\pmvA]}) < 0 \\
%   0  & \mathit{min}(\gain{\pmvA}{\txT[\pmvA]}) \geq 0
% \end{cases}
% \]
% We write that $\txT[\pmvA]$ is \emph{minimally} executed in $\confG\rightarrow^{\txT[\pmvA]}\confGi$ if $\mathit{ext}(\txT[\pmvA]) = -\gain[\confG]{\pmvA}{\txT[\pmvA]}$.
% Furthermore, we note that for
% $\confG \myxrightarrow{\actAmmSwap{\pmvA}{d}{\_}{\tokT[0]}{\_}{\tokT[1]}} \confGi$
% to be minimally executed, the following constraints on the reserves of the AMM pair $(\ammR[0]:\tokT[0],\ammR[1]:\tokT[1])\in\confG$
% must be satisfied.

% \bartnote{I do not understand the statement of the theorem below}

% \albertonote{My understanding is that this section tries to establish a bound on the maximum extractable value for miner / the solution to the one of the mining games. However, I my intuition is that the bound is too coarse as it considers the maximum extractable value from user transactions in states that may not be reachable at all (e.g. reachable only via deposits/redeems to push the pairs/curves in the ideal situation - for the miner) so the bound may not be interesting if we are restricting to swap actions in the miner. Can these bounds be computed efficiently? If yes, then I could see some potential use of the result. Otherwise, I don't know. I understand that the ext for minted tokens can be computed (arbitrage) but I don't see how this can be done for user transactions.}

% \begin{theorem}
%   \label{thm:optimal-miner-gain}
%   \jamesnote{Assumption: unbounded blocksize.}
%   Let $\TxT$ be a multiset of users' transactions, and
%   let $\confG$ be any blockchain state. Then,
%   \[
%   \sum_{\txT \in \TxT} \mathit{ext}(\txT) + \sum_{(\_:\tokT[0],\_:\tokT[1])\in\confG} \mathit{ext}^{\confG}(\tokT[0],\tokT[1])
%   \; \geq \;
%   \mev{\confG}{\TxT}
%   \]
% \end{theorem}


%        %        \jamesnote{Proof sketch below.}
%        %        \begin{proof}
%        %        Consider a run $\confG[0] \myxrightarrow{\bcB} \confGi$ where (1) $\bcB \in S_{\bcB}$, includes all unprofitable $\txT[\pmvA] \in S_{\pmvA}$ and (2) for all
%        %        $(\ammR[0]:\tokT[0],\ammR[1]:\tokT[1]) \in \confGi$, $\ammR[1]/\ammR[0] = \exchOInit(\tokT[0])/\exchOInit(\tokT[1])$. We show that $\gain[{\confG[0]}]{\pmvA}{\bcB}$ must decrease by relaxing (1) or (2). Thus, the maximum miner gain must be $\gain[{\confG[0]}]{\pmvM}{\bcB} = -\gain[{\confG[0]}]{\pmvA}{\bcB}$ (wealth conservation), which is equal to $\gain[{\confGi[0]}]{\pmvA}{\bcBi}$ in~\Cref{thm:optimal-miner-gain}.
%        %        \end{proof}


% \albertonote{We can also say that the problem is decidable and provide the na\"ive brute-force algorithm we discussed (which exploits some of the properties of the above theorem), correct?}

% \albertonote{If, hypothetically, we get the theorem right and the algorithm as well (see sketch above) - how would they play together?}

% \HSL


% \subsection{Step minimization}

% \jamesnote{Here, only include tx with negative gain.}

% \albertonote{My understanding of this section is that we want to quantify the number of swap operations that the miner needs to ``execute'' the optimal solution to the MEV-extraction problem. Correct? Given an actual solution $\lambda$ the problem is trivial, right?}

% \albertonote{Isn't $k$ fixed already for the entire paper?}


% We write $\textsf{step}_{k}(\txT) = \big((\ammR[i]^0,\ammR[j]^0),(\ammR[i]^1,\ammR[j]^1)\big)$ where \mbox{$(\ammR[i]^0:\tokT[i],\ammR[j]^0:\tokT[j]) \in \confG[0]$} and \mbox{$(\ammR[i]^1:\tokT[i],\ammR[j]^1:\tokT[j]) \in \confG[1]$} for the minimized swap step $\confG[0] \rightarrow^{\txT} \confG[1]$. Here, $\textsf{step}_{k}^{0}(\txT) = (\ammR[0]^0,\ammR[1]^0)$, and $\textsf{step}_{k}^{1}(\txT) = (\ammR[0]^1,\ammR[1]^1)$.

% For a set of transactions $S=\{\txT,\txTi,\cdots \}$ we write
% \begin{equation}
%   \begin{split}
%     &\textsf{heads}_{k}(S,\tokT[0],\tokT[1]) = \{ (r,i) \mid
%     \circled{0} \wedge \circled{1} \wedge \circled{2}
%     \wedge \circled{3}
%     \}
%     \\
%     &\circled{0}\:\txT \in S
%     \quad
%     \circled{1}\:\txLab(\txT) = \ammSwapOp(\_:\tokT[0],\_:\tokT[1])
%     \\
%     &\circled{2}\:\textsf{head}_{k}(\txT) = r
%     \quad
%     \circled{3}\:i(\txT) = i
%   \end{split}
% \end{equation}

% Similarly for $\textsf{tails}_{k}(S,\tokT[0],\tokT[1])$. We define
% the multiset
% \begin{equation}
%   \begin{array}{c}
%     \textsf{coHeads}_{k}(S,\tokT[0],\tokT[1]) = \{ r^{\min(n,m)} \mid
%     \circled{0} \wedge \circled{1} \wedge\circled{2}
%     \wedge \circled{3} \}
%     \\[3pt]
%     \circled{0}\: (r,i) \in \textsf{heads}_{k}(S,\tokT[0],\tokT[1])
%     \quad
%     \circled{1}\: \exists (r',i') \in \textsf{tails}_{k}(S,\tokT[0],\tokT[1]) : r = r'
%     \\[3pt]
%     \circled{2}\: n = \: \mid \{ (r'',i'') \mid (r'',i'') \in \textsf{heads}_{k}(S,\tokT[0],\tokT[1]) \wedge r'' = r \} \mid
%     \\[3pt]
%     \circled{3}\: m = \: \mid \{ (r''',i''') \mid (r''',i''') \in \textsf{tails}_{k}(S,\tokT[0],\tokT[1]) \wedge r''' = r \} \mid
%   \end{array}
% \end{equation}

% \begin{theorem}[Minimized steps]
%   \label{thm:min-steps}

%   Let $\confG = (\ammR[0]:\tokT[0],\ammR[1]:\tokT[1]) \mid \cdots$ and $S_{\pmvA}$ be a set of \emph{unprofitable} user transactions. $\pmvM$ can execute $\confG \rightarrow^{\bcB} \confGi$ to extract an optimal gain where
%   \albertonote{what follows are not boolean predicates so I don't understand the ``where ...'' part. Do you mean how to quantify the minimum number of steps that the miner needs?}
%   \begin{itemize}
%   \item $\mid \textsf{heads}_{k}(S_{\pmvA},\tokT[0],\tokT[1]) \mid -(\sum_{r^n}^{\textsf{coHeads}_{k}(S_{\pmvA},\tokT[0],\tokT[1])} n) + 1$ steps if
%     \[
%     \not\exists (r,i) \in \textsf{effHeads}_{k}(S_{\pmvA},\tokT[0],\tokT[1]) : r = (\ammR[0],\ammR[1])
%     \]
%   \item $\mid \textsf{heads}_{k}(S_{\pmvA},\tokT[0],\tokT[1]) \mid -(\sum_{r^n}^{\textsf{coHeads}_{k}(S_{\pmvA},\tokT[0],\tokT[1])} n)$ steps otherwise
%   \end{itemize}
% \end{theorem}


% \subsection{Miner liquidity}

% \albertonote{My understanding of this section is that we want to quantify the funds that the miner needs to ``execute'' the optimal solution to the MEV-extraction problem. Correct? Given an actual solution $\lambda$ the problem is trivial, right?}


% We denote $\mathit{liq}_{k}^{\tokT[0],\tokT[1]}(\ammR[i],\ammRi[i],\tokT[i])$ as the change in user balance (or liquidity) when performing a swap from $\confG = (\ammR[0]:\tokT[0],\ammR[1]:\tokT[1])\mid \cdots$ to $\confGi = (\ammRi[0]:\tokT[0],\ammRi[1]:\tokT[1])\mid \cdots$ with a single step, where $k=\ammR[0]\cdot\ammR[1]$.
% \begin{equation}
%   \mathit{liq}_{k}^{\tokT[0],\tokT[1]}(\ammR,\ammRi,\tokT[i])
%   = \big((\ammR - \ammRi):\tokT[i], (k/\ammR - k/\ammRi):\tokT[1-i]\big)
% \end{equation}

% We denote miner liquidity as the minimum miner balances in $\confG$ to execute $\confG \rightarrow^{\bcB}\confGi$.

% \begin{lemma}[Minimum liquidity]
%   \label{lma:min-liquidity}
%   Let $\confG = (\ammR[0]:\tokT[0],\ammR[1]:\tokT[1]) \mid \cdots$, $\txT[\pmvA] = \actAmmSwapL{\pmvA}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}$ and
%   $k=\ammR[0]\cdot\ammR[1]$.
%   Extracting optimal miner value in $\confG \rightarrow^{\bcB} \confGi$ where $act_{\pmvA}(\bcB) = \{\txT\}$ requires $liq_{k}^{\tokT[0],\tokT[1]}(\ammR[0],\mathit{left}(step_{k}^{0}(\txT)),\tokT[0])+liq_{k}^{\tokT[0],\tokT[1]}(\mathit{left}(step_{k}^{1}(\txT)),\ammR[0],\tokT[0])$ of miner liquidity in $\confG$.
% \end{lemma}

% \jamesnote{TODO: ...}


